Algorithm as Experiment: Machine Learning, Market Design, and Policy Eligibility Rules

Algorithms make a growing portion of policy and business decisions. We develop a treatment-effect estimator using algorithmic decisions as instruments for a class of stochastic and deterministic algorithms. Our estimator is consistent and asymptotically normal for well-defined causal effects. A special case of our setup is multidimensional regression discontinuity designs with complex boundaries. We apply our estimator to evaluate the Coronavirus Aid, Relief, and Economic Security Act, which allocated many billions of dollars worth of relief funding to hospitals via an algorithmic rule. The funding is shown to have little effect on COVID-19-related hospital activities. Naive estimates exhibit selection bias.

==> miscellaneous/tables/2SLS_safety_net_county_a.tex <==
\begin{table}[h] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Estimated Effects of Funding on County Utilization}
{\scriptsize
\begin{tabularx}{\textwidth}{lCCCCCCCCCC}

\hline\hline\tabularnewline[-1.8ex]
{}&{OLS with}&{OLS with}&{2SLS with}&\multicolumn{7}{c}{Our Method: 2SLS with Approximate Propensity Score Controls} \tabularnewline
{}&{No}&{Covariate}&{No} \tabularnewline[-1.8ex]\cline{5-11} \tabularnewline[-1.0ex]
{}&{Controls}&{Controls}&{Controls}&{ $\delta = 0.01$}&{ $\delta = 0.025$}&{ $\delta = 0.05$}&{ $\delta = 0.075$}&{ $\delta = 0.1$}&{ $\delta = 0.25$}&{ $\delta = 0.5$} \tabularnewline
&(1)&(2)&(3)&(4)&(5)&(6)&(7)&(8)&(9)&(10)\\
\midrule\addlinespace[1.5ex]
\multicolumn{11}{l}{\# Confirmed/Suspected COVID Patients}\tabularnewline \midrule\addlinespace[1.5ex]
First stage&&&18.42***&9.85**&7.39***&5.50***&5.48***&4.66***&4.48***&4.06*** \tabularnewline
(in millions \$)&&&(1.43)&(4.69)&(2.13)&(1.76)&(1.33)&(1.19)&(0.87)&(0.76) \tabularnewline
\$1mm of funding&26.07***&25.75***&21.88***&26.90**&23.94&1.62&$-$0.23&$-$19.01&$-$27.85**&$-$44.48*** \tabularnewline
&(4.86)&(5.01)&(2.43)&(12.68)&(19.72)&(23.36)&(15.67)&(15.92)&(11.16)&(13.65) \tabularnewline
N&2473&2473&2473&56&151&294&392&524&1004&1276 \tabularnewline
\midrule\addlinespace[1.5ex] \multicolumn{11}{l}{\# Confirmed COVID Patients}\tabularnewline \midrule\addlinespace[1.5ex]
First stage&&&18.42***&9.85**&7.39***&5.50***&5.48***&4.66***&4.48***&4.06*** \tabularnewline
(in millions \$)&&&(1.43)&(4.69)&(2.13)&(1.76)&(1.33)&(1.19)&(0.87)&(0.76) \tabularnewline
\$1mm of funding&19.66***&19.35***&17.38***&19.77*&27.39&16.62&9.24&$-$7.25&$-$19.93**&$-$32.92*** \tabularnewline
&(4.33)&(4.46)&(2.17)&(10.68)&(16.69)&(16.40)&(11.06)&(10.57)&(8.62)&(10.64) \tabularnewline
N&2473&2473&2473&56&151&294&392&524&1004&1276 \tabularnewline
\midrule\addlinespace[1.5ex] \multicolumn{11}{l}{\# Confirmed/Suspected COVID Patients in ICU}\tabularnewline \midrule\addlinespace[1.5ex]
First stage&&&18.42***&9.85**&7.39***&5.50***&5.48***&4.66***&4.48***&4.06*** \tabularnewline
(in millions \$)&&&(1.43)&(4.69)&(2.13)&(1.76)&(1.33)&(1.19)&(0.87)&(0.76) \tabularnewline
\$1mm of funding&7.16***&7.03***&6.57***&9.57**&13.32**&4.40&1.54&$-$3.02&$-$7.65**&$-$12.13*** \tabularnewline
&(1.32)&(1.36)&(0.71)&(3.74)&(5.90)&(5.85)&(4.22)&(4.36)&(3.36)&(3.88) \tabularnewline
N&2473&2473&2473&56&151&294&392&524&1004&1276 \tabularnewline
\midrule\addlinespace[1.5ex] \multicolumn{11}{l}{\# Confirmed COVID Patients in ICU}\tabularnewline \midrule\addlinespace[1.5ex]
First stage&&&18.42***&9.85**&7.39***&5.50***&5.48***&4.66***&4.48***&4.06*** \tabularnewline
(in millions \$)&&&(1.43)&(4.69)&(2.13)&(1.76)&(1.33)&(1.19)&(0.87)&(0.76) \tabularnewline
\$1mm of funding&6.15***&6.03***&5.69***&8.38**&13.28**&5.12&1.48&$-$3.37&$-$7.66**&$-$11.23*** \tabularnewline
&(1.28)&(1.32)&(0.68)&(3.53)&(5.62)&(5.37)&(3.82)&(3.93)&(3.09)&(3.54) \tabularnewline
N&2473&2473&2473&56&151&294&392&524&1004&1276 \tabularnewline
\bottomrule \addlinespace[1.5ex]

\end{tabularx}
\begin{flushleft}
{\it Notes}: In this table we regress relevant outcomes at the county level on safety net funding. Column 1 presents the results of OLS regression of the outcome variables on safety net funding without any controls. Column 2 presents the results of OLS regression of the outcome variables on safety net funding controlling for disproportionate patient percentage, uncompensated care per bed and profit margin.  In columns 3--10, we instrument safety net funding with eligibility to receive this funding and present the results of 2SLS regressions. In columns 3--10, the first stage shows the effect of being deemed eligible on the amount of relief funding received by counties, in millions of dollars. Column 3 shows the results of a 2SLS regression with no controls.  In columns 4--10, we run this regression controlling for the Approximate Propensity Score with different values of bandwidth $\delta$ on the sample with nondegenerate Approximate Propensity Scores.  All Approximate Propensity Scores are computed by averaging 10,000 simulation draws. The outcome variables are the 7 day totals for the week spanning July 31st, 2020 to August 6th, 2020. Confirmed or Suspected COVID patients refer to the sum of patients in inpatient beds with lab-confirmed/suspected COVID-19. Confirmed COVID patients refer to the sum of patients in inpatient beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Inpatient bed totals also include observation beds. Similarly, Confirmed/Suspected COVID patients in ICU refer to the sum of patients in ICU beds with lab-confirmed or suspected COVID-19. Confirmed COVID patients in ICU refers to the sum of patients in ICU beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Robust standard errors are reported in parentheses. */**/*** indicate $p <$ 0.10/0.05/0.01
\end{flushleft}
}
\label{table:2sls_safetynet_CA}
\end{table}


==> miscellaneous/tables/2SLS_safety_net_county_a_fs.tex <==
\begin{table}[h] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Estimated Effects of Funding on County Utilization}
{\scriptsize
\begin{tabularx}{\textwidth}{lCCCCCCCCCC}

\toprule
&{(1)}&{(2)}&{(3)}&{(4)}&{(5)}&{(6)}&{(7)}&{(8)}&{(9)}&{(10)} \tabularnewline
{}&{}&{}&{}&\multicolumn{7}{c}{Our Method: 2SLS with Approximate Propensity Score Controls} \tabularnewline {}&{OLS with}&{OLS with}&{2SLS with}&\tabularnewline[-2ex] \cline{5-11} \tabularnewline
{}&{No Controls}&{Covariate Controls}&{No Controls}&{ $\delta = 0.01$}&{ $\delta = 0.025$}&{ $\delta = 0.05$}&{ $\delta = 0.075$}&{ $\delta = 0.1$}&{ $\delta = 0.25$}&{ $\delta = 0.5$} \tabularnewline
\midrule\addlinespace[1.5ex]
\multicolumn{11}{l}{\# Confirmed/Suspected COVID Patients}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&18.42***&8.30**&6.92***&5.83***&6.37***&7.24***&8.51***&8.98*** \tabularnewline
(in millions \$)&&&(1.43)&(3.43)&(1.76)&(1.69)&(1.33)&(1.26)&(0.83)&(0.66) \tabularnewline
\$1mm of funding&26.07***&25.75***&21.88***&$-$10.18&11.42&7.18&9.97&7.09&5.11*&4.73* \tabularnewline
&(4.86)&(5.01)&(2.43)&(11.26)&(11.16)&(16.44)&(10.86)&(7.18)&(3.00)&(2.43) \tabularnewline
N&2473&2473&2473&56&152&294&392&524&1004&1276 \tabularnewline
\midrule\addlinespace[1.5ex] \multicolumn{11}{l}{\# Confirmed COVID Patients}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&18.42***&8.30**&6.92***&5.83***&6.37***&7.24***&8.51***&8.98*** \tabularnewline
(in millions \$)&&&(1.43)&(3.43)&(1.76)&(1.69)&(1.33)&(1.26)&(0.83)&(0.66) \tabularnewline
\$1mm of funding&19.66***&19.35***&17.38***&$-$14.03&16.76*&20.43*&16.75**&11.01**&5.49**&5.12** \tabularnewline
&(4.33)&(4.46)&(2.17)&(11.08)&(9.43)&(11.07)&(7.68)&(5.11)&(2.58)&(2.27) \tabularnewline
N&2473&2473&2473&56&152&294&392&524&1004&1276 \tabularnewline
\midrule\addlinespace[1.5ex] \multicolumn{11}{l}{\# Confirmed/Suspected COVID Patients in ICU}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&18.42***&8.30**&6.92***&5.83***&6.37***&7.24***&8.51***&8.98*** \tabularnewline
(in millions \$)&&&(1.43)&(3.43)&(1.76)&(1.69)&(1.33)&(1.26)&(0.83)&(0.66) \tabularnewline
\$1mm of funding&7.16***&7.03***&6.57***&$-$1.57&9.61***&6.11*&4.66*&4.06**&1.90**&1.96*** \tabularnewline
&(1.32)&(1.36)&(0.71)&(3.31)&(3.56)&(3.37)&(2.43)&(1.80)&(0.91)&(0.73) \tabularnewline
N&2473&2473&2473&56&152&294&392&524&1004&1276 \tabularnewline
\midrule\addlinespace[1.5ex] \multicolumn{11}{l}{\# Confirmed COVID Patients in ICU}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&18.42***&8.30**&6.92***&5.83***&6.37***&7.24***&8.51***&8.98*** \tabularnewline
(in millions \$)&&&(1.43)&(3.43)&(1.76)&(1.69)&(1.33)&(1.26)&(0.83)&(0.66) \tabularnewline
\$1mm of funding&6.15***&6.03***&5.69***&$-$2.29&9.86***&6.49**&4.17*&3.10**&1.12&1.25* \tabularnewline
&(1.28)&(1.32)&(0.68)&(3.48)&(3.50)&(3.20)&(2.22)&(1.54)&(0.80)&(0.67) \tabularnewline
N&2473&2473&2473&56&152&294&392&524&1004&1276 \tabularnewline
\bottomrule \addlinespace[1.5ex]

\end{tabularx}

}
\end{table}


==> miscellaneous/tables/2SLS_safety_net_county_b.tex <==
\begin{table}[h] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Estimated Effects of Funding on County Outcomes}
{\scriptsize
\begin{tabularx}{\textwidth}{lCCCCCCCCCC}

\hline\hline\tabularnewline[-1.8ex]
{}&{OLS with}&{OLS with}&{2SLS with}&\multicolumn{7}{c}{Our Method: 2SLS with Approximate Propensity Score Controls} \tabularnewline
{}&{No}&{Covariate}&{No} \tabularnewline[-1.8ex]\cline{5-11} \tabularnewline[-1.0ex]
{}&{Controls}&{Controls}&{Controls}&{ $\delta = 0.01$}&{ $\delta = 0.025$}&{ $\delta = 0.05$}&{ $\delta = 0.075$}&{ $\delta = 0.1$}&{ $\delta = 0.25$}&{ $\delta = 0.5$} \tabularnewline
&(1)&(2)&(3)&(4)&(5)&(6)&(7)&(8)&(9)&(10)\\
\midrule\addlinespace[1.5ex]
\multicolumn{11}{l}{\# COVID Cases}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&18.42***&9.79**&7.38***&5.52***&5.49***&4.64***&4.50***&4.11*** \tabularnewline
(in millions \$)&&&(1.43)&(4.62)&(2.14)&(1.75)&(1.30)&(1.17)&(0.87)&(0.75) \tabularnewline
\$1mm of funding&18.19***&17.85***&15.31***&21.03**&22.31**&11.04&$-$0.46&$-$16.39&$-$26.87***&$-$36.37*** \tabularnewline
&(3.58)&(3.68)&(1.72)&(10.24)&(10.85)&(11.52)&(10.64)&(11.70)&(9.34)&(9.80) \tabularnewline
N&2467&2467&2467&56&152&294&392&524&1003&1276 \tabularnewline
\midrule\addlinespace[1.5ex] \multicolumn{11}{l}{\# COVID Deaths}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&18.42***&9.79**&7.38***&5.52***&5.49***&4.64***&4.50***&4.11*** \tabularnewline
(in millions \$)&&&(1.43)&(4.62)&(2.14)&(1.75)&(1.30)&(1.17)&(0.87)&(0.75) \tabularnewline
\$1mm of funding&0.38***&0.37***&0.36***&0.28&0.75&0.40&0.15&$-$0.28&$-$0.60***&$-$0.87*** \tabularnewline
&(0.10)&(0.10)&(0.05)&(0.30)&(0.50)&(0.45)&(0.32)&(0.29)&(0.21)&(0.24) \tabularnewline
N&2467&2467&2467&56&152&294&392&524&1003&1276 \tabularnewline
\bottomrule \addlinespace[1.5ex]

\end{tabularx}
\begin{flushleft}
{\it Notes}: In this table we regress relevant outcomes at the county level on safety net funding. Column 1 presents the results of OLS regression of the outcome variables on safety net funding without any controls. Column 2 presents the results of OLS regression of the outcome variables on safety net funding controlling for disproportionate patient percentage, uncompensated care per bed and profit margin.  In columns 3--10, we instrument safety net funding with eligibility to receive this funding and present the results of 2SLS regressions. In columns 3--10, the first stage shows the effect of being deemed eligible on the amount of relief funding received by counties, in millions of dollars. Column 3 shows the results of a 2SLS regression with no controls.  In columns 4--10, we run this regression controlling for the Approximate Propensity Score with different values of bandwidth $\delta$ on the sample with nondegenerate Approximate Propensity Scores.  All Approximate Propensity Scores are computed by averaging 10,000 simulation draws. The outcome variables are the 7 day totals for the week spanning August 13st, 2020 to August 20th, 2020. Robust standard errors are reported in parentheses. */**/*** indicate p < 0.10/0.05/0.01
\end{flushleft}
}
\label{table:2sls_safetynet_CB}
\end{table}


==> miscellaneous/tables/2SLS_safety_net_county_b_fs.tex <==
\begin{table}[h] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Estimated Effects of Funding on County Outcomes}
{\scriptsize
\begin{tabularx}{\textwidth}{lCCCCCCCCCC}

\toprule
&{(1)}&{(2)}&{(3)}&{(4)}&{(5)}&{(6)}&{(7)}&{(8)}&{(9)}&{(10)} \tabularnewline
{}&{}&{}&{}&\multicolumn{7}{c}{Our Method: 2SLS with Approximate Propensity Score Controls} \tabularnewline {}&{OLS with}&{OLS with}&{2SLS with}&\tabularnewline[-2ex] \cline{5-11} \tabularnewline
{}&{No Controls}&{Covariate Controls}&{No Controls}&{ $\delta = 0.01$}&{ $\delta = 0.025$}&{ $\delta = 0.05$}&{ $\delta = 0.075$}&{ $\delta = 0.1$}&{ $\delta = 0.25$}&{ $\delta = 0.5$} \tabularnewline
\midrule\addlinespace[1.5ex]
\multicolumn{11}{l}{\# COVID Cases}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&17.10***&8.30**&6.92***&5.83***&6.37***&7.42***&8.49***&8.93*** \tabularnewline
(in millions \$)&&&(1.29)&(3.43)&(1.76)&(1.69)&(1.33)&(1.24)&(0.82)&(0.66) \tabularnewline
\$1mm of funding&24.82***&24.45***&17.93***&$-$8.44&28.54**&24.06*&14.01&5.67&$-$2.79&$-$2.91 \tabularnewline
&(4.84)&(5.00)&(2.01)&(11.67)&(13.67)&(12.89)&(9.07)&(6.12)&(3.70)&(2.71) \tabularnewline
N&2456&2456&2456&56&152&294&392&523&1002&1274 \tabularnewline
\midrule\addlinespace[1.5ex] \multicolumn{11}{l}{\# COVID Deaths}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&17.10***&8.30**&6.92***&5.83***&6.37***&7.42***&8.49***&8.93*** \tabularnewline
(in millions \$)&&&(1.29)&(3.43)&(1.76)&(1.69)&(1.33)&(1.24)&(0.82)&(0.66) \tabularnewline
\$1mm of funding&0.49***&0.48***&0.40***&$-$0.40&0.41&0.31&0.17&0.04&$-$0.06&$-$0.06 \tabularnewline
&(0.12)&(0.13)&(0.05)&(0.27)&(0.34)&(0.29)&(0.20)&(0.14)&(0.07)&(0.06) \tabularnewline
N&2456&2456&2456&56&152&294&392&523&1002&1274  \tabularnewline
\bottomrule \addlinespace[1.5ex]

\end{tabularx}

}
\end{table}


==> miscellaneous/tables/2SLS_safety_net_county_sa.tex <==
\begin{table}[h] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Estimated Effects of Funding on County Utilization}
{\scriptsize
\begin{tabularx}{\textwidth}{lCCCCCCCCCC}

\toprule
&{(1)}&{(2)}&{(3)}&{(4)}&{(5)}&{(6)}&{(7)}&{(8)}&{(9)}&{(10)} \tabularnewline
{}&{}&{}&{}&\multicolumn{7}{c}{Our Method: 2SLS with Approximate Propensity Score Controls} \tabularnewline {}&{OLS with}&{OLS with}&{2SLS with}&\tabularnewline[-2ex] \cline{5-11} \tabularnewline
{}&{No Controls}&{Covariate Controls}&{No Controls}&{ $\delta = 0.005$}&{ $\delta = 0.01$}&{ $\delta = 0.015$}&{ $\delta = 0.02$}&{ $\delta = 0.03$}&{ $\delta = 0.04$}&{ $\delta = 0.05$} \tabularnewline
\midrule\addlinespace[1.5ex]
\multicolumn{11}{l}{\# Confirmed/Suspected COVID Patients}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&18.42***&7.80**&9.82**&7.52**&7.42***&7.76***&7.27***&5.62*** \tabularnewline
(in millions \$)&&&(1.43)&(3.50)&(4.70)&(3.56)&(2.58)&(1.94)&(1.62)&(1.78) \tabularnewline
\$1mm of funding&26.07***&25.75***&21.88***&39.16***&24.33*&35.82**&42.24*&17.77&5.56&1.70 \tabularnewline
&(4.86)&(5.01)&(2.43)&(14.82)&(13.14)&(18.27)&(22.65)&(18.30)&(19.15)&(22.89) \tabularnewline
N&2473&2473&2473&24&56&79&121&178&231&294 \tabularnewline
\midrule\addlinespace[1.5ex] \multicolumn{11}{l}{\# Confirmed COVID Patients}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&18.42***&7.80**&9.82**&7.52**&7.42***&7.76***&7.27***&5.62*** \tabularnewline
(in millions \$)&&&(1.43)&(3.50)&(4.70)&(3.56)&(2.58)&(1.94)&(1.62)&(1.78) \tabularnewline
\$1mm of funding&19.66***&19.35***&17.38***&23.51**&17.18&31.97**&34.50*&24.68*&16.31&16.39 \tabularnewline
&(4.33)&(4.46)&(2.17)&(9.80)&(11.38)&(15.44)&(18.34)&(14.63)&(13.57)&(16.00) \tabularnewline
N&2473&2473&2473&24&56&79&121&178&231&294 \tabularnewline
\midrule\addlinespace[1.5ex] \multicolumn{11}{l}{\# Confirmed/Suspected COVID Patients in ICU}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&18.42***&7.80**&9.82**&7.52**&7.42***&7.76***&7.27***&5.62*** \tabularnewline
(in millions \$)&&&(1.43)&(3.50)&(4.70)&(3.56)&(2.58)&(1.94)&(1.62)&(1.78) \tabularnewline
\$1mm of funding&7.16***&7.03***&6.57***&8.58**&8.69**&12.82**&14.99**&10.23**&5.24&4.53 \tabularnewline
&(1.32)&(1.36)&(0.71)&(3.75)&(3.94)&(5.25)&(6.26)&(5.10)&(4.89)&(5.73) \tabularnewline
N&2473&2473&2473&24&56&79&121&178&231&294 \tabularnewline
\midrule\addlinespace[1.5ex] \multicolumn{11}{l}{\# Confirmed COVID Patients in ICU}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&18.42***&7.80**&9.82**&7.52**&7.42***&7.76***&7.27***&5.62*** \tabularnewline
(in millions \$)&&&(1.43)&(3.50)&(4.70)&(3.56)&(2.58)&(1.94)&(1.62)&(1.78) \tabularnewline
\$1mm of funding&6.15***&6.03***&5.69***&5.92&7.53**&11.89**&14.22**&10.54**&5.98&5.11 \tabularnewline
&(1.28)&(1.32)&(0.68)&(3.86)&(3.77)&(4.83)&(5.83)&(4.79)&(4.47)&(5.25) \tabularnewline
N&2473&2473&2473&24&56&79&121&178&231&294 \tabularnewline
\bottomrule \addlinespace[1.5ex]

\end{tabularx}
\begin{flushleft}
\footnotesize {\it Notes}: In this table we regress relevant outcomes at the county level on safety net funding. Column 1 presents the results of OLS regression of the outcome variables on safety net funding without any controls. Column 2 presents the results of OLS regression of the outcome variables on safety net funding controlling for disproportionate patient percentage, uncompensated care per bed and profit margin.  In columns 3--10, we instrument safety net funding with eligibility to receive this funding and present the results of 2SLS regressions. In columns 3--10, the first stage shows the effect of being deemed eligible on the amount of relief funding received by counties, in millions of dollars. Column 3 shows the results of a 2SLS regression with no controls.  In columns 4--10, we run this regression controlling for the Approximate Propensity Score with different values of bandwidth $\delta$ on the sample with nondegenerate Approximate Propensity Scores.  All Approximate Propensity Scores are computed by averaging 10,000 simulation draws. The outcome variables are the 7 day totals for the week spanning July 31st, 2020 to August 6th, 2020. Confirmed or Suspected COVID patients refer to the sum of patients in inpatient beds with lab-confirmed/suspected COVID-19. Confirmed COVID patients refer to the sum of patients in inpatient beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Inpatient bed totals also include observation beds. Similarly, Confirmed/Suspected COVID patients in ICU refer to the sum of patients in ICU beds with lab-confirmed or suspected COVID-19. Confirmed COVID patients in ICU refers to the sum of patients in ICU beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Robust standard errors are reported in parentheses. */**/*** indicate p < 0.10/0.05/0.01
\end{flushleft}
}
\end{table}


==> miscellaneous/tables/2SLS_safety_net_county_sb.tex <==
\begin{table}[h] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Estimated Effects of Funding on County Outcomes}
{\scriptsize
\begin{tabularx}{\textwidth}{lCCCCCCCCCC}

\toprule
&{(1)}&{(2)}&{(3)}&{(4)}&{(5)}&{(6)}&{(7)}&{(8)}&{(9)}&{(10)} \tabularnewline
{}&{}&{}&{}&\multicolumn{7}{c}{Our Method: 2SLS with Approximate Propensity Score Controls} \tabularnewline {}&{OLS with}&{OLS with}&{2SLS with}&\tabularnewline[-2ex] \cline{5-11} \tabularnewline
{}&{No Controls}&{Covariate Controls}&{No Controls}&{ $\delta = 0.005$}&{ $\delta = 0.01$}&{ $\delta = 0.015$}&{ $\delta = 0.02$}&{ $\delta = 0.03$}&{ $\delta = 0.04$}&{ $\delta = 0.05$} \tabularnewline
\midrule\addlinespace[1.5ex]
\multicolumn{11}{l}{\# COVID Cases}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&17.10***&7.80**&9.82**&7.52**&7.42***&7.76***&7.27***&5.62*** \tabularnewline
(in millions \$)&&&(1.29)&(3.50)&(4.70)&(3.56)&(2.58)&(1.94)&(1.62)&(1.78) \tabularnewline
\$1mm of funding&24.82***&24.45***&17.93***&36.54*&22.07&34.64*&47.28**&37.35**&24.47*&19.56 \tabularnewline
&(4.84)&(5.00)&(2.01)&(22.21)&(14.24)&(18.74)&(23.68)&(17.04)&(14.14)&(17.00) \tabularnewline
N&2456&2456&2456&24&56&79&121&178&231&294 \tabularnewline
\midrule\addlinespace[1.5ex] \multicolumn{11}{l}{\# COVID Deaths}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&17.10***&7.80**&9.82**&7.52**&7.42***&7.76***&7.27***&5.62*** \tabularnewline
(in millions \$)&&&(1.29)&(3.50)&(4.70)&(3.56)&(2.58)&(1.94)&(1.62)&(1.78) \tabularnewline
\$1mm of funding&0.49***&0.48***&0.40***&0.07&0.22&0.44&0.66&0.58&0.35&0.21 \tabularnewline
&(0.12)&(0.13)&(0.05)&(0.19)&(0.30)&(0.42)&(0.48)&(0.38)&(0.33)&(0.39) \tabularnewline
N&2456&2456&2456&24&56&79&121&178&231&294 \tabularnewline
\bottomrule \addlinespace[1.5ex]

\end{tabularx}
\begin{flushleft}
\footnotesize {\it Notes}: In this table we regress relevant outcomes at the county level on safety net funding. Column 1 presents the results of OLS regression of the outcome variables on safety net funding without any controls. Column 2 presents the results of OLS regression of the outcome variables on safety net funding controlling for disproportionate patient percentage, uncompensated care per bed and profit margin.  In columns 3--10, we instrument safety net funding with eligibility to receive this funding and present the results of 2SLS regressions. In columns 3--10, the first stage shows the effect of being deemed eligible on the amount of relief funding received by counties, in millions of dollars. Column 3 shows the results of a 2SLS regression with no controls.  In columns 4--10, we run this regression controlling for the Approximate Propensity Score with different values of bandwidth $\delta$ on the sample with nondegenerate Approximate Propensity Scores.  All Approximate Propensity Scores are computed by averaging 10,000 simulation draws. The outcome variables are the 7 day totals for the week spanning August 13st, 2020 to August 20th, 2020. Robust standard errors are reported in parentheses. */**/*** indicate p < 0.10/0.05/0.01
\end{flushleft}
}
\end{table}


==> miscellaneous/tables/2SLS_safety_net_dist.tex <==
\begin{table}[h] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Estimated Effects of Funding on Hospital Utilization}
{\scriptsize
\begin{tabularx}{\textwidth}{lCCCCCCCCCCC}

\toprule
{}&{}&{}&{}&\multicolumn{8}{c}{RD with Linear Boundary Distance Controls} \tabularnewline {}&{OLS with}&{OLS with}&{2SLS with}&\tabularnewline[-2ex] \cline{5-12} \tabularnewline
{}&{No Controls}&{Covariate Controls}&{No Controls}&{ $\delta = 0.01$}&{ $\delta = 0.025$}&{ $\delta = 0.05$}&{ $\delta = 0.075$}&{ $\delta = 0.1$}&{ $\delta = 0.25$}&{ $\delta = CCT$}&{ $\delta = IK$} \tabularnewline
&{(1)}&{(2)}&{(3)}&{(4)}&{(5)}&{(6)}&{(7)}&{(8)}&{(9)}&{(10)}&{(11)} \tabularnewline
\midrule\addlinespace[1.5ex]
\multicolumn{11}{l}{\# Confirmed/Suspected COVID Patients}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&&& \tabularnewline
First stage&&&13.78***&14.65**&13.48***&14.28***&14.30***&13.88***&14.07***&14.06***&14.13*** \tabularnewline
(in millions \$)&&&(0.49)&(5.68)&(3.13)&(2.13)&(1.72)&(1.45)&(0.96)&(0.94)&(0.94) \tabularnewline
\$1mm of funding&5.58***&3.25***&2.77***&-0.53&-2.83&-2.34&-3.11&-1.99&0.47&1.14&1.21 \tabularnewline
&(0.68)&(0.89)&(0.58)&(5.16)&(4.37)&(4.53)&(3.94)&(3.34)&(1.83)&(1.81)&(1.81) \tabularnewline
N&3532&3532&3532&74&195&394&553&725&1395&1437&1429 \tabularnewline
\midrule\addlinespace[1.5ex] \multicolumn{11}{l}{\# Confirmed COVID Patients}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&&& \tabularnewline
First stage&&&13.90***&15.83**&14.38***&15.04***&14.90***&14.39***&14.17***&14.17***&14.24*** \tabularnewline
(in millions \$)&&&(0.50)&(6.10)&(3.34)&(2.19)&(1.76)&(1.49)&(0.98)&(0.96)&(0.96) \tabularnewline
\$1mm of funding&4.53***&2.50***&2.44***&0.68&-2.02&1.46&0.25&0.29&0.61&1.26&1.32 \tabularnewline
&(0.63)&(0.79)&(0.50)&(3.88)&(3.43)&(2.02)&(1.86)&(1.63)&(1.14)&(1.17)&(1.17) \tabularnewline
N&3558&3558&3558&72&191&387&545&716&1373&1415&1407 \tabularnewline
\midrule\addlinespace[1.5ex] \multicolumn{11}{l}{\# Confirmed/Suspected COVID Patients in ICU}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&&& \tabularnewline
First stage&&&13.88***&14.23**&13.93***&16.07***&15.46***&14.74***&14.51***&14.50***&14.58*** \tabularnewline
(in millions \$)&&&(0.51)&(5.77)&(3.26)&(2.27)&(1.86)&(1.57)&(1.01)&(0.99)&(0.99) \tabularnewline
\$1mm of funding&1.67***&0.91***&0.95***&1.04&0.43&0.31&0.00&0.29&0.18&0.36&0.42 \tabularnewline
&(0.21)&(0.28)&(0.18)&(1.37)&(1.08)&(0.69)&(0.66)&(0.58)&(0.41)&(0.42)&(0.42) \tabularnewline
N&3445&3445&3445&73&186&376&526&686&1321&1361&1355 \tabularnewline
\midrule\addlinespace[1.5ex] \multicolumn{11}{l}{\# Confirmed COVID Patients in ICU}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&&& \tabularnewline
First stage&&&13.89***&14.94**&14.01***&15.86***&15.47***&14.86***&14.45***&14.47***&14.54*** \tabularnewline
(in millions \$)&&&(0.50)&(5.90)&(3.31)&(2.25)&(1.85)&(1.56)&(1.01)&(0.99)&(0.99) \tabularnewline
\$1mm of funding&1.51***&0.82***&0.88***&0.55&-0.17&0.07&0.08&0.22&0.15&0.35&0.39 \tabularnewline
&(0.21)&(0.27)&(0.17)&(1.45)&(1.17)&(0.66)&(0.61)&(0.54)&(0.39)&(0.39)&(0.40) \tabularnewline
N&3503&3503&3503&69&181&372&520&678&1327&1370&1362 \tabularnewline
\bottomrule \addlinespace[1.5ex]

\end{tabularx}
\begin{flushleft}
{\it Notes}: In this table we regress relevant outcomes at the hospital level on safety net funding. Column 1 presents the results of OLS regression of the outcome variables on safety net funding without any controls. Column 2 presents the results of OLS regression of the outcome variables on safety net funding controlling for disproportionate patient percentage, uncompensated care per bed and profit margin.  In columns 3--11, we instrument safety net funding with eligibility to receive this funding and present the results of 2SLS regressions. In columns 3--11, the first stage shows the effect of being deemed eligible on the amount of relief funding received by hospitals, in millions of dollars. Column 3 shows the results of a 2SLS regression with no controls. In columns 4--11, we run this regression linearly controlling for the boundary distance and using different values of bandwidth $\delta$. Column 10 uses the Calonico, Cattaneo and Titiunik (2014) optimal MSE bandwidth computed for the funding variable. Column 11 uses the Imbens and Kalyanaraman (2012) optimal MSE bandwidth computed for the funding variable. The outcome variables are the 7 day totals for the week spanning July 31st, 2020 to August 6th, 2020. Confirmed or Suspected COVID patients refer to the sum of patients in inpatient beds with lab-confirmed/suspected COVID-19. Confirmed COVID patients refer to the sum of patients in inpatient beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Inpatient bed totals also include observation beds. Similarly, Confirmed/Suspected COVID patients in ICU refer to the sum of patients in ICU beds with lab-confirmed or suspected COVID-19. Confirmed COVID patients in ICU refers to the sum of patients in ICU beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Robust standard errors are reported in parentheses. */**/*** indicate p < 0.10/0.05/0.01
\end{flushleft}
}
\end{table}


==> miscellaneous/tables/2SLS_safety_net_fs.tex <==
\begin{table}[h] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Estimated Effects of Funding on Hospital Utilization}
{\scriptsize
\begin{tabularx}{\textwidth}{lCCCCCCCCCC}

\toprule
&{(1)}&{(2)}&{(3)}&{(4)}&{(5)}&{(6)}&{(7)}&{(8)}&{(9)}&{(10)} \tabularnewline
{}&{}&{}&{}&\multicolumn{7}{c}{Our Method: 2SLS with Approximate Propensity Score Controls} \tabularnewline {}&{OLS with}&{OLS with}&{2SLS with}&\tabularnewline[-2ex] \cline{5-11} \tabularnewline
{}&{No Controls}&{Covariate Controls}&{No Controls}&{ $\delta = 0.01$}&{ $\delta = 0.025$}&{ $\delta = 0.05$}&{ $\delta = 0.075$}&{ $\delta = 0.1$}&{ $\delta = 0.25$}&{ $\delta = 0.5$} \tabularnewline
\midrule\addlinespace[1.5ex]
\multicolumn{11}{l}{\# Confirmed/Suspected COVID Patients}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&13.78***&11.33***&13.74***&15.04***&14.78***&14.29***&14.12***&13.50*** \tabularnewline
(in millions \$)&&&(0.49)&(3.16)&(2.31)&(1.72)&(1.39)&(1.19)&(0.75)&(0.58) \tabularnewline
\$1mm of funding&5.58***&3.25***&2.77***&$-$4.91&$-$1.38&$-$2.26&$-$3.32&$-$2.37&0.43&0.79 \tabularnewline
&(0.68)&(0.89)&(0.58)&(6.82)&(4.33)&(4.53)&(4.17)&(3.30)&(1.47)&(1.01) \tabularnewline
N&3532&3532&3532&73&195&392&547&719&1389&1947 \tabularnewline
\midrule\addlinespace[1.5ex] \multicolumn{11}{l}{\# Confirmed COVID Patients}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&13.90***&11.78***&14.52***&15.55***&15.28***&14.70***&14.26***&13.61*** \tabularnewline
(in millions \$)&&&(0.50)&(3.36)&(2.41)&(1.75)&(1.41)&(1.21)&(0.76)&(0.59) \tabularnewline
\$1mm of funding&4.53***&2.50***&2.44***&$-$3.18&$-$1.99&1.74&0.51&0.22&0.13&0.23 \tabularnewline
&(0.63)&(0.79)&(0.50)&(5.83)&(3.16)&(1.96)&(1.75)&(1.55)&(1.04)&(0.82) \tabularnewline
N&3558&3558&3558&70&191&385&539&709&1366&1923 \tabularnewline
\midrule\addlinespace[1.5ex] \multicolumn{11}{l}{\# Confirmed/Suspected COVID Patients in ICU}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&13.88***&10.47***&13.48***&15.71***&15.55***&14.86***&14.46***&13.71*** \tabularnewline
(in millions \$)&&&(0.51)&(3.11)&(2.33)&(1.75)&(1.43)&(1.23)&(0.78)&(0.60) \tabularnewline
\$1mm of funding&1.67***&0.91***&0.95***&0.27&0.72&0.35&0.02&0.19&0.04&0.10 \tabularnewline
&(0.21)&(0.28)&(0.18)&(2.13)&(1.13)&(0.68)&(0.63)&(0.56)&(0.38)&(0.31) \tabularnewline
N&3445&3445&3445&72&186&374&520&678&1314&1846 \tabularnewline
\midrule\addlinespace[1.5ex] \multicolumn{11}{l}{\# Confirmed COVID Patients in ICU}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&13.89***&11.02***&14.50***&16.30***&16.05***&15.29***&14.56***&13.83*** \tabularnewline
(in millions \$)&&&(0.50)&(3.41)&(2.50)&(1.83)&(1.49)&(1.27)&(0.80)&(0.61) \tabularnewline
\$1mm of funding&1.51***&0.82***&0.88***&$-$0.22&0.08&0.28&0.17&0.18&$-$0.08&$-$0.06 \tabularnewline
&(0.21)&(0.27)&(0.17)&(2.24)&(1.10)&(0.63)&(0.57)&(0.52)&(0.37)&(0.29) \tabularnewline
N&3503&3503&3503&67&181&370&514&671&1321&1868 \tabularnewline
\bottomrule \addlinespace[1.5ex]

\end{tabularx}

}
\end{table}


==> miscellaneous/tables/2SLS_safety_net_indicator_10.tex <==
\begin{table}[h] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Estimated Effects of Funding on Hospital Utilization}
{\scriptsize
\begin{tabularx}{\linewidth}{lCCCCCCCCCC}

\hline\hline\tabularnewline[-1.8ex]
{}&{OLS with}&{OLS with}&{2SLS with}&\multicolumn{7}{c}{Our Method: 2SLS with Approximate Propensity Score Controls} \tabularnewline
{}&{No}&{Covariate}&{No} \tabularnewline[-1.8ex]\cline{5-11} \tabularnewline[-1.8ex]
{}&{Controls}&{Controls}&{Controls}&{ $\delta = 0.01$}&{ $\delta = 0.025$}&{ $\delta = 0.05$}&{ $\delta = 0.075$}&{ $\delta = 0.1$}&{ $\delta = 0.25$}&{ $\delta = 0.5$} \tabularnewline
&(1)&(2)&(3)&(4)&(5)&(6)&(7)&(8)&(9)&(10)\\
\midrule\addlinespace[1.5ex]
\multicolumn{11}{l}{\# Confirmed/Suspected COVID Patients}\tabularnewline 
\midrule\addlinespace[1.5ex]
First stage&&&0.42***&0.30*&0.34***&0.39***&0.38***&0.37***&0.41***&0.39*** \tabularnewline
&&&(0.02)&(0.18)&(0.12)&(0.08)&(0.07)&(0.06)&(0.04)&(0.03) \tabularnewline
> \$10mm funding&150.82***&90.04***&91.22***&$-$50.94&$-$73.30&$-$112.64&$-$150.62&$-$110.33&5.02&$-$10.45 \tabularnewline
&(15.43)&(19.82)&(19.07)&(283.57)&(214.76)&(182.25)&(169.64)&(136.88)&(54.31)&(40.31) \tabularnewline
N&3532&3532&3532&73&195&392&547&719&1389&1947 \tabularnewline
\midrule\addlinespace[1.5ex] 
\multicolumn{11}{l}{\# Confirmed COVID Patients}\tabularnewline 
\midrule\addlinespace[1.5ex] \tabularnewline
First stage&&&0.42***&0.35*&0.40***&0.43***&0.41***&0.39***&0.41***&0.40*** \tabularnewline
&&&(0.02)&(0.19)&(0.12)&(0.08)&(0.07)&(0.06)&(0.04)&(0.03) \tabularnewline
> \$10mm funding&127.41***&75.95***&80.67***&2.41&$-$76.82&49.63&4.75&$-$0.99&$-$3.13&$-$20.83 \tabularnewline
&(14.08)&(17.32)&(16.53)&(202.58)&(143.63)&(75.69)&(70.83)&(63.99)&(38.55)&(32.19) \tabularnewline
N&3558&3558&3558&70&191&385&539&709&1366&1923 \tabularnewline
\midrule\addlinespace[1.5ex] 
\multicolumn{11}{l}{\# Confirmed/Suspected COVID Patients in ICU}\tabularnewline 
\midrule\addlinespace[1.5ex] 
First stage&&&0.42***&0.29*&0.36***&0.46***&0.44***&0.41***&0.43***&0.40*** \tabularnewline
&&&(0.02)&(0.17)&(0.11)&(0.08)&(0.07)&(0.06)&(0.04)&(0.03) \tabularnewline
> \$10mm funding&46.99***&27.52***&31.14***&47.19&26.74&12.34&$-$1.89&5.63&$-$1.06&$-$10.48 \tabularnewline
&(4.95)&(6.38)&(6.04)&(72.38)&(47.41)&(25.11)&(24.41)&(21.47)&(13.42)&(11.83) \tabularnewline
N&3445&3445&3445&72&186&374&520&678&1314&1846 \tabularnewline
\midrule\addlinespace[1.5ex] 
\multicolumn{11}{l}{\# Confirmed COVID Patients in ICU}\tabularnewline 
\midrule\addlinespace[1.5ex]
First stage&&&0.43***&0.33*&0.38***&0.46***&0.45***&0.43***&0.44***&0.41*** \tabularnewline
&&&(0.02)&(0.19)&(0.12)&(0.09)&(0.07)&(0.06)&(0.04)&(0.03) \tabularnewline
> \$10mm funding&41.62***&23.91***&28.37***&24.31&$-$4.01&6.01&1.44&4.36&$-$4.44&$-$11.29 \tabularnewline
&(4.79)&(5.94)&(5.65)&(72.70)&(49.11)&(23.85)&(22.12)&(19.64)&(12.89)&(10.99) \tabularnewline
N&3503&3503&3503&67&181&370&514&671&1321&1868 \tabularnewline
\bottomrule

\end{tabularx}
\caption*{
\scriptsize{\it Notes}: In this table we regress outcomes at the hospital level on a indicator for receiving more than \$10mm in safety net funding. Column 1 presents the results of OLS regression without controls. Column 2 presents the results of OLS controlling for disproportionate patient percentage, uncompensated care per bed, and profit margin.  In columns 3$-$10, we instrument the funding indicator with eligibility to receive this funding and present the results of 2SLS regressions. In columns 3$-$10, the first stage shows the effect of funding eligibility on the funding indicator. Column 3 shows the results of a 2SLS regression with no controls.  In columns 4$-$10, we control for the Approximate Propensity Score with different values of bandwidth $\delta$ on the sample with nondegenerate Approximate Propensity Scores. All Approximate Propensity Scores are computed by averaging 10,000 simulation draws. The outcome variables are the 7 day totals for the week spanning July 31st, 2020 to August 6th, 2020. Confirmed or Suspected COVID patients refer to the sum of patients in inpatient beds with lab-confirmed/suspected COVID-19. Confirmed COVID patients refer to the sum of patients in inpatient beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Inpatient bed totals also include observation beds. Similarly, Confirmed/Suspected COVID patients in ICU refer to the sum of patients in ICU beds with lab-confirmed or suspected COVID-19. Confirmed COVID patients in ICU refers to the sum of patients in ICU beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Robust standard errors are reported in parentheses. */**/*** indicate p < 0.10/0.05/0.01
}
\label{table:2sls_safetynet_indicator10}
}
\end{table}


==> miscellaneous/tables/2SLS_safety_net_indicator_20.tex <==
\begin{table}[h] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Estimated Effects of Funding on Hospital Utilization (> 20mm Indicator)}
{\scriptsize
\begin{tabularx}{\linewidth}{lCCCCCCCCCC}

\toprule
&{(1)}&{(2)}&{(3)}&{(4)}&{(5)}&{(6)}&{(7)}&{(8)}&{(9)}&{(10)} \tabularnewline \midrule
{}&{}&{}&{}&\multicolumn{7}{c}{Our Method: 2SLS with Approximate Propensity Score Controls} \tabularnewline {}&{OLS with}&{OLS with}&{2SLS with}&\tabularnewline[-2ex] \cline{5-11} \tabularnewline
{}&{No Controls}&{Covariate Controls}&{No Controls}&{ $\delta = 0.01$}&{ $\delta = 0.025$}&{ $\delta = 0.05$}&{ $\delta = 0.075$}&{ $\delta = 0.1$}&{ $\delta = 0.25$}&{ $\delta = 0.5$} \tabularnewline
\midrule \addlinespace[\belowrulesep]
\multicolumn{11}{l}{\# Confirmed/Suspected COVID Patients}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&0.20***&0.22&0.24**&0.22***&0.21***&0.20***&0.20***&0.18*** \tabularnewline
&&&(0.02)&(0.17)&(0.10)&(0.07)&(0.06)&(0.05)&(0.03)&(0.02) \tabularnewline
> \$20mm funding&213.92***&130.58***&189.25***&$-$70.10&$-$103.98&$-$198.25&$-$273.67&$-$200.19&10.27&$-$22.66 \tabularnewline
&(27.02)&(31.05)&(38.92)&(395.80)&(306.68)&(326.32)&(318.05)&(254.86)&(110.87)&(87.82) \tabularnewline
N&3532&3532&3532&73&195&392&547&719&1389&1947 \tabularnewline
\midrule\addlinespace[1.5ex] \multicolumn{11}{l}{\# Confirmed COVID Patients}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&0.21***&0.26&0.26**&0.24***&0.22***&0.21***&0.20***&0.18*** \tabularnewline
&&&(0.02)&(0.18)&(0.11)&(0.07)&(0.06)&(0.05)&(0.03)&(0.02) \tabularnewline
> \$20mm funding&170.51***&98.58***&165.56***&3.32&$-$119.44&89.75&8.79&$-$1.86&$-$6.33&$-$45.16 \tabularnewline
&(24.66)&(27.58)&(33.77)&(279.62)&(227.72)&(137.04)&(130.70)&(119.72)&(78.00)&(70.34) \tabularnewline
N&3558&3558&3558&70&191&385&539&709&1366&1923 \tabularnewline
\midrule\addlinespace[1.5ex] \multicolumn{11}{l}{\# Confirmed/Suspected COVID Patients in ICU}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&0.20***&0.21&0.24**&0.25***&0.23***&0.21***&0.20***&0.18*** \tabularnewline
&&&(0.02)&(0.16)&(0.10)&(0.07)&(0.06)&(0.05)&(0.03)&(0.02) \tabularnewline
> \$20mm funding&65.65***&39.31***&64.41***&64.90&40.37&23.17&$-$3.60&10.94&$-$2.25&$-$23.29 \tabularnewline
&(8.80)&(10.10)&(12.36)&(96.40)&(71.06)&(46.79)&(46.60)&(41.48)&(28.45)&(26.67) \tabularnewline
N&3445&3445&3445&72&186&374&520&678&1314&1846 \tabularnewline
\midrule\addlinespace[1.5ex] \multicolumn{11}{l}{\# Confirmed COVID Patients in ICU}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&0.20***&0.24&0.24**&0.24***&0.23***&0.22***&0.21***&0.19*** \tabularnewline
&&&(0.02)&(0.18)&(0.11)&(0.07)&(0.06)&(0.05)&(0.03)&(0.02) \tabularnewline
> \$20mm funding&58.53***&34.83***&59.58***&33.47&$-$6.36&11.41&2.76&8.49&$-$9.38&$-$25.18 \tabularnewline
&(8.67)&(9.67)&(11.77)&(97.86)&(78.18)&(45.13)&(42.24)&(38.08)&(27.38)&(24.89) \tabularnewline
N&3503&3503&3503&67&181&370&514&671&1321&1868 \tabularnewline
\bottomrule \addlinespace[\belowrulesep]

\end{tabularx}
\begin{flushleft}
\tiny {\it Notes}: In this table we regress relevant outcomes at the hospital level on a safety net funding indicator. Column 1 presents the results of OLS regression of the outcome variables on the safety net funding indicator without any controls. Column 2 presents the results of OLS regression of the outcome variables on the safety net funding indicator controlling for disproportionate patient percentage, uncompensated care per bed and profit margin.  In columns 3$-$10, we instrument the safety net funding indicator with eligibility to receive this funding and present the results of 2SLS regressions. In columns 3$-$10, the first stage shows the effect of being deemed eligible on the amount of relief funding received by hospitals, in millions of dollars. Column 3 shows the results of a 2SLS regression with no controls.  In columns 4$-$10, we run this regression controlling for the Approximate Propensity Score with different values of bandwidth $\delta$ on the sample with nondegenerate Approximate Propensity Scores.  All Approximate Propensity Scores are computed by averaging 10,000 simulation draws. The outcome variables are the 7 day totals for the week spanning July 31st, 2020 to August 6th, 2020. Confirmed or Suspected COVID patients refer to the sum of patients in inpatient beds with lab-confirmed/suspected COVID-19. Confirmed COVID patients refer to the sum of patients in inpatient beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Inpatient bed totals also include observation beds. Similarly, Confirmed/Suspected COVID patients in ICU refer to the sum of patients in ICU beds with lab-confirmed or suspected COVID-19. Confirmed COVID patients in ICU refers to the sum of patients in ICU beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Robust standard errors are reported in parentheses. */**/*** indicate p < 0.10/0.05/0.01
\end{flushleft}
}
\end{table}


==> miscellaneous/tables/2SLS_safety_net_indicator_30.tex <==
\begin{table}[h] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Estimated Effects of Funding on Hospital Utilization (> 30mm Indicator)}
{\scriptsize
\begin{tabularx}{\linewidth}{lCCCCCCCCCC}

\toprule
&{(1)}&{(2)}&{(3)}&{(4)}&{(5)}&{(6)}&{(7)}&{(8)}&{(9)}&{(10)} \tabularnewline \midrule
{}&{}&{}&{}&\multicolumn{7}{c}{Our Method: 2SLS with Approximate Propensity Score Controls} \tabularnewline {}&{OLS with}&{OLS with}&{2SLS with}&\tabularnewline[-2ex] \cline{5-11} \tabularnewline
{}&{No Controls}&{Covariate Controls}&{No Controls}&{ $\delta = 0.01$}&{ $\delta = 0.025$}&{ $\delta = 0.05$}&{ $\delta = 0.075$}&{ $\delta = 0.1$}&{ $\delta = 0.25$}&{ $\delta = 0.5$} \tabularnewline
\midrule \addlinespace[\belowrulesep]
\multicolumn{11}{l}{\# Confirmed/Suspected COVID Patients}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&0.13***&0.14&0.09&0.13**&0.13***&0.14***&0.13***&0.12*** \tabularnewline
&&&(0.01)&(0.13)&(0.08)&(0.05)&(0.05)&(0.04)&(0.03)&(0.02) \tabularnewline
> \$30mm funding&243.64***&142.70***&291.49***&$-$114.54&$-$270.96&$-$334.81&$-$451.39&$-$298.41&15.23&$-$35.24 \tabularnewline
&(36.05)&(40.87)&(61.01)&(636.18)&(838.19)&(559.43)&(538.92)&(385.37)&(164.27)&(137.03) \tabularnewline
N&3532&3532&3532&73&195&392&547&719&1389&1947 \tabularnewline
\midrule\addlinespace[1.5ex] \multicolumn{11}{l}{\# Confirmed COVID Patients}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&0.13***&0.16&0.10&0.14**&0.14***&0.14***&0.14***&0.12*** \tabularnewline
&&&(0.01)&(0.14)&(0.08)&(0.06)&(0.05)&(0.04)&(0.03)&(0.02) \tabularnewline
> \$30mm funding&181.52***&92.89***&255.01***&5.47&$-$302.93&150.92&14.43&$-$2.77&$-$9.38&$-$70.21 \tabularnewline
&(32.42)&(35.86)&(53.77)&(460.91)&(628.29)&(231.41)&(214.35)&(178.61)&(115.68)&(110.19) \tabularnewline
N&3558&3558&3558&70&191&385&539&709&1366&1923 \tabularnewline
\midrule\addlinespace[1.5ex] \multicolumn{11}{l}{\# Confirmed/Suspected COVID Patients in ICU}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&0.13***&0.13&0.09&0.16***&0.15***&0.15***&0.14***&0.12*** \tabularnewline
&&&(0.01)&(0.13)&(0.08)&(0.06)&(0.05)&(0.04)&(0.03)&(0.02) \tabularnewline
> \$30mm funding&66.54***&34.06***&98.11***&105.92&104.83&36.32&$-$5.62&15.79&$-$3.27&$-$35.15 \tabularnewline
&(10.78)&(12.45)&(19.72)&(191.65)&(196.88)&(74.13)&(72.65)&(59.83)&(41.36)&(40.60) \tabularnewline
N&3445&3445&3445&72&186&374&520&678&1314&1846 \tabularnewline
\midrule\addlinespace[1.5ex] \multicolumn{11}{l}{\# Confirmed COVID Patients in ICU}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&0.13***&0.15&0.09&0.16***&0.15***&0.15***&0.14***&0.12*** \tabularnewline
&&&(0.01)&(0.14)&(0.09)&(0.06)&(0.05)&(0.04)&(0.03)&(0.02) \tabularnewline
> \$30mm funding&58.35***&28.93**&91.12***&54.75&$-$17.66&17.99&4.32&12.14&$-$13.77&$-$38.13 \tabularnewline
&(10.59)&(11.92)&(18.88)&(176.48)&(218.24)&(71.54)&(66.06)&(54.41)&(40.31)&(38.10) \tabularnewline
N&3503&3503&3503&67&181&370&514&671&1321&1868 \tabularnewline
\bottomrule \addlinespace[\belowrulesep]

\end{tabularx}
\begin{flushleft}
\tiny {\it Notes}: In this table we regress relevant outcomes at the hospital level on a safety net funding indicator. Column 1 presents the results of OLS regression of the outcome variables on the safety net funding indicator without any controls. Column 2 presents the results of OLS regression of the outcome variables on the safety net funding indicator controlling for disproportionate patient percentage, uncompensated care per bed and profit margin.  In columns 3$-$10, we instrument the safety net funding indicator with eligibility to receive this funding and present the results of 2SLS regressions. In columns 3$-$10, the first stage shows the effect of being deemed eligible on the amount of relief funding received by hospitals, in millions of dollars. Column 3 shows the results of a 2SLS regression with no controls.  In columns 4$-$10, we run this regression controlling for the Approximate Propensity Score with different values of bandwidth $\delta$ on the sample with nondegenerate Approximate Propensity Scores.  All Approximate Propensity Scores are computed by averaging 10,000 simulation draws. The outcome variables are the 7 day totals for the week spanning July 31st, 2020 to August 6th, 2020. Confirmed or Suspected COVID patients refer to the sum of patients in inpatient beds with lab-confirmed/suspected COVID-19. Confirmed COVID patients refer to the sum of patients in inpatient beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Inpatient bed totals also include observation beds. Similarly, Confirmed/Suspected COVID patients in ICU refer to the sum of patients in ICU beds with lab-confirmed or suspected COVID-19. Confirmed COVID patients in ICU refers to the sum of patients in ICU beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Robust standard errors are reported in parentheses. */**/*** indicate p < 0.10/0.05/0.01
\end{flushleft}
}
\end{table}


==> miscellaneous/tables/2SLS_safety_net_indicator_40.tex <==
\begin{table}[h] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Estimated Effects of Funding on Hospital Utilization (> 40mm Indicator)}
{\scriptsize
\begin{tabularx}{\linewidth}{lCCCCCCCCCC}

\toprule
&{(1)}&{(2)}&{(3)}&{(4)}&{(5)}&{(6)}&{(7)}&{(8)}&{(9)}&{(10)} \tabularnewline \midrule
{}&{}&{}&{}&\multicolumn{7}{c}{Our Method: 2SLS with Approximate Propensity Score Controls} \tabularnewline {}&{OLS with}&{OLS with}&{2SLS with}&\tabularnewline[-2ex] \cline{5-11} \tabularnewline
{}&{No Controls}&{Covariate Controls}&{No Controls}&{ $\delta = 0.01$}&{ $\delta = 0.025$}&{ $\delta = 0.05$}&{ $\delta = 0.075$}&{ $\delta = 0.1$}&{ $\delta = 0.25$}&{ $\delta = 0.5$} \tabularnewline
\midrule \addlinespace[\belowrulesep]
\multicolumn{11}{l}{\# Confirmed/Suspected COVID Patients}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&0.08***&0.17&0.07&0.11**&0.12***&0.13***&0.10***&0.07*** \tabularnewline
&&&(0.01)&(0.13)&(0.08)&(0.05)&(0.04)&(0.03)&(0.02)&(0.02) \tabularnewline
> \$40mm funding&274.97***&165.30***&497.25***&$-$89.02&$-$339.95&$-$407.15&$-$478.69&$-$308.75&21.03&$-$56.74 \tabularnewline
&(52.24)&(55.24)&(110.39)&(488.89)&(1,080.25)&(683.07)&(563.51)&(393.55)&(226.85)&(220.72) \tabularnewline
N&3532&3532&3532&73&195&392&547&719&1389&1947 \tabularnewline
\midrule\addlinespace[1.5ex] \multicolumn{11}{l}{\# Confirmed COVID Patients}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&0.08***&0.19&0.08&0.12**&0.13***&0.13***&0.10***&0.07*** \tabularnewline
&&&(0.01)&(0.14)&(0.08)&(0.05)&(0.04)&(0.04)&(0.02)&(0.02) \tabularnewline
> \$40mm funding&218.57***&124.76**&435.01***&4.37&$-$379.98&184.02&15.47&$-$2.89&$-$12.92&$-$112.93 \tabularnewline
&(49.04)&(50.58)&(96.41)&(368.06)&(827.86)&(285.71)&(230.16)&(186.32)&(159.33)&(177.73) \tabularnewline
N&3558&3558&3558&70&191&385&539&709&1366&1923 \tabularnewline
\midrule\addlinespace[1.5ex] \multicolumn{11}{l}{\# Confirmed/Suspected COVID Patients in ICU}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&0.08***&0.17&0.07&0.13**&0.13***&0.14***&0.10***&0.07*** \tabularnewline
&&&(0.01)&(0.12)&(0.08)&(0.05)&(0.04)&(0.04)&(0.02)&(0.02) \tabularnewline
> \$40mm funding&71.81***&36.50**&168.75***&81.94&131.52&44.04&$-$6.14&16.87&$-$4.63&$-$58.12 \tabularnewline
&(15.83)&(16.87)&(36.74)&(142.01)&(255.55)&(90.58)&(79.37)&(64.22)&(58.50)&(67.48) \tabularnewline
N&3445&3445&3445&72&186&374&520&678&1314&1846 \tabularnewline
\midrule\addlinespace[1.5ex] \multicolumn{11}{l}{\# Confirmed COVID Patients in ICU}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&0.08***&0.19&0.07&0.13**&0.14***&0.14***&0.10***&0.08*** \tabularnewline
&&&(0.01)&(0.14)&(0.08)&(0.05)&(0.04)&(0.04)&(0.02)&(0.02) \tabularnewline
> \$40mm funding&68.09***&37.53**&158.06***&42.74&$-$22.17&21.66&4.67&13.10&$-$18.91&$-$60.72 \tabularnewline
&(15.87)&(16.40)&(34.97)&(136.11)&(275.12)&(86.42)&(71.41)&(58.94)&(55.19)&(60.95) \tabularnewline
N&3503&3503&3503&67&181&370&514&671&1321&1868 \tabularnewline
\bottomrule \addlinespace[\belowrulesep]

\end{tabularx}
\begin{flushleft}
\tiny {\it Notes}: In this table we regress relevant outcomes at the hospital level on a safety net funding indicator. Column 1 presents the results of OLS regression of the outcome variables on the safety net funding indicator without any controls. Column 2 presents the results of OLS regression of the outcome variables on the safety net funding indicator controlling for disproportionate patient percentage, uncompensated care per bed and profit margin.  In columns 3$-$10, we instrument the safety net funding indicator with eligibility to receive this funding and present the results of 2SLS regressions. In columns 3$-$10, the first stage shows the effect of being deemed eligible on the amount of relief funding received by hospitals, in millions of dollars. Column 3 shows the results of a 2SLS regression with no controls.  In columns 4$-$10, we run this regression controlling for the Approximate Propensity Score with different values of bandwidth $\delta$ on the sample with nondegenerate Approximate Propensity Scores.  All Approximate Propensity Scores are computed by averaging 10,000 simulation draws. The outcome variables are the 7 day totals for the week spanning July 31st, 2020 to August 6th, 2020. Confirmed or Suspected COVID patients refer to the sum of patients in inpatient beds with lab-confirmed/suspected COVID-19. Confirmed COVID patients refer to the sum of patients in inpatient beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Inpatient bed totals also include observation beds. Similarly, Confirmed/Suspected COVID patients in ICU refer to the sum of patients in ICU beds with lab-confirmed or suspected COVID-19. Confirmed COVID patients in ICU refers to the sum of patients in ICU beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Robust standard errors are reported in parentheses. */**/*** indicate p < 0.10/0.05/0.01
\end{flushleft}
}
\end{table}


==> miscellaneous/tables/2SLS_safety_net_mid.tex <==
\begin{table}[h] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Estimated Effects of Funding on Hospital Utilization}
{\scriptsize
\begin{tabularx}{\textwidth}{lCCCCCCCCCC}

\toprule
&{(1)}&{(2)}&{(3)}&{(4)}&{(5)}&{(6)}&{(7)}&{(8)}&{(9)}&{(10)} \tabularnewline
{}&{}&{}&{}&\multicolumn{7}{c}{Our Method: 2SLS with Approximate Propensity Score Controls} \tabularnewline {}&{OLS with}&{OLS with}&{2SLS with}&\tabularnewline[-2ex] \cline{5-11} \tabularnewline
{}&{No Controls}&{Covariate Controls}&{No Controls}&{ $\delta = 0.01$}&{ $\delta = 0.025$}&{ $\delta = 0.05$}&{ $\delta = 0.075$}&{ $\delta = 0.1$}&{ $\delta = 0.25$}&{ $\delta = 0.5$} \tabularnewline
\midrule\addlinespace[1.5ex]
\multicolumn{11}{l}{\# Confirmed/Suspected COVID Patients}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&16.33***&13.56***&15.02***&15.67***&15.46***&15.80***&15.93***&15.26*** \tabularnewline
(in millions \$)&&&(0.55)&(4.56)&(2.89)&(1.95)&(1.64)&(1.44)&(0.96)&(0.73) \tabularnewline
\$1mm of funding&5.13***&2.43**&4.56***&-1.03&2.66&-2.25&-2.95&-1.09&2.50&2.48** \tabularnewline
&(0.65)&(0.96)&(0.59)&(7.43)&(5.79)&(5.25)&(4.81)&(3.59)&(1.56)&(1.16) \tabularnewline
N&3267&3267&3267&54&149&310&443&598&1177&1696 \tabularnewline
\midrule\addlinespace[1.5ex] \multicolumn{11}{l}{\# Confirmed COVID Patients}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&16.39***&13.36***&15.39***&16.06***&15.81***&16.06***&16.06***&15.36*** \tabularnewline
(in millions \$)&&&(0.55)&(4.55)&(2.89)&(1.96)&(1.64)&(1.45)&(0.97)&(0.73) \tabularnewline
\$1mm of funding&3.97***&1.69**&3.73***&-0.47&0.11&2.10&1.16&1.25&1.74*&1.54* \tabularnewline
&(0.53)&(0.78)&(0.51)&(6.06)&(3.83)&(2.30)&(1.88)&(1.54)&(1.03)&(0.91) \tabularnewline
N&3301&3301&3301&53&148&306&438&589&1159&1678 \tabularnewline
\midrule\addlinespace[1.5ex] \multicolumn{11}{l}{\# Confirmed/Suspected COVID Patients in ICU}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&16.49***&13.54***&15.52***&16.35***&16.14***&16.39***&16.30***&15.50*** \tabularnewline
(in millions \$)&&&(0.57)&(4.44)&(2.84)&(1.97)&(1.65)&(1.47)&(0.99)&(0.75) \tabularnewline
\$1mm of funding&1.58***&0.71**&1.54***&0.75&1.72&0.88&0.59&0.89&0.67*&0.57* \tabularnewline
&(0.20)&(0.30)&(0.19)&(1.88)&(1.25)&(0.81)&(0.70)&(0.58)&(0.38)&(0.34) \tabularnewline
N&3190&3190&3190&54&148&301&426&568&1110&1604 \tabularnewline
\midrule\addlinespace[1.5ex] \multicolumn{11}{l}{\# Confirmed COVID Patients in ICU}\tabularnewline \midrule\addlinespace[1.5ex]&&&&&&&&&& \tabularnewline
First stage&&&16.50***&14.89***&15.82***&16.63***&16.51***&16.79***&16.55***&15.77*** \tabularnewline
(in millions \$)&&&(0.56)&(4.82)&(2.95)&(2.02)&(1.72)&(1.50)&(1.02)&(0.76) \tabularnewline
\$1mm of funding&1.38***&0.59**&1.36***&0.55&0.84&0.68&0.67&0.78&0.47&0.39 \tabularnewline
&(0.19)&(0.27)&(0.18)&(1.89)&(1.30)&(0.77)&(0.63)&(0.53)&(0.36)&(0.32) \tabularnewline
N&3249&3249&3249&49&140&296&418&557&1119&1628 \tabularnewline
\bottomrule \addlinespace[1.5ex]

\end{tabularx}
\begin{flushleft}
\tiny {\it Notes}: In this table we regress relevant outcomes at the hospital level on safety net funding. Column 1 presents the results of OLS regression of the outcome variables on safety net funding without any controls. Column 2 presents the results of OLS regression of the outcome variables on safety net funding controlling for disproportionate patient percentage, uncompensated care per bed and profit margin.  In columns 3--10, we instrument safety net funding with eligibility to receive this funding and present the results of 2SLS regressions. In columns 3--10, the first stage shows the effect of being deemed eligible on the amount of relief funding received by hospitals, in millions of dollars. Column 3 shows the results of a 2SLS regression with no controls.  In columns 4--10, we run this regression controlling for the Approximate Propensity Score with different values of bandwidth $\delta$ on the sample with nondegenerate Approximate Propensity Scores.  All Approximate Propensity Scores are computed by averaging 10,000 simulation draws. The outcome variables are the 7 day totals for the week spanning July 31st, 2020 to August 6th, 2020. Confirmed or Suspected COVID patients refer to the sum of patients in inpatient beds with lab-confirmed/suspected COVID-19. Confirmed COVID patients refer to the sum of patients in inpatient beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Inpatient bed totals also include observation beds. Similarly, Confirmed/Suspected COVID patients in ICU refer to the sum of patients in ICU beds with lab-confirmed or suspected COVID-19. Confirmed COVID patients in ICU refers to the sum of patients in ICU beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Robust standard errors are reported in parentheses. */**/*** indicate p < 0.10/0.05/0.01
\end{flushleft}
}
\end{table}


==> miscellaneous/tables/2sls_safety_net_combined_indicator.tex <==
\begin{table}[h] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Effects of Funding on Hospital Behavior}
{\scriptsize
\begin{tabularx}{\linewidth}{lCCCCCCCCCC}

\hline\hline\tabularnewline[-1.8ex]
{}&{OLS with}&{OLS with}&{2SLS with}&\multicolumn{7}{c}{Our Method: 2SLS with Approximate Propensity Score Controls} \tabularnewline
{}&{No}&{Covariate}&{No} \tabularnewline[-1.8ex]\cline{5-11} \tabularnewline[-1.8ex]
{}&{Controls}&{Controls}&{Controls}&{ $\delta = 0.01$}&{ $\delta = 0.025$}&{ $\delta = 0.05$}&{ $\delta = 0.075$}&{ $\delta = 0.1$}&{ $\delta = 0.25$}&{ $\delta = 0.5$} \tabularnewline
&(1)&(2)&(3)&(4)&(5)&(6)&(7)&(8)&(9)&(10)\\
\midrule\addlinespace[1.5ex]
\multicolumn{11}{l}{\# Confirmed COVID Patients}\tabularnewline 
\midrule\addlinespace[1.5ex]
Reduced Form&&&33.97***&8.82&$-$31.57&25.21&15.28&10.63&9.17&5.23 \tabularnewline
&&&(7.44)&(66.76)&(54.25)&(34.19)&(30.38)&(25.91)&(15.96)&(12.41) \tabularnewline
First stage&&&0.42***&0.35*&0.40***&0.43***&0.41***&0.39***&0.41***&0.40*** \tabularnewline
&&&(0.02)&(0.19)&(0.12)&(0.08)&(0.07)&(0.06)&(0.04)&(0.03) \tabularnewline
> \$10mm funding&127.4***&76.0***&80.67***&2.41&$-$76.82&49.63&4.75&$-$0.99&$-$3.13&$-$20.83 \tabularnewline
&(14.08)&(17.32)&(16.53)&(202.58)&(143.63)&(75.69)&(70.83)&(63.99)&(38.55)&(32.19) \tabularnewline
N&3558&3558&3558&70&191&385&539&709&1366&1923 \tabularnewline
\midrule\addlinespace[1.5ex] 
\multicolumn{11}{l}{\# Confirmed COVID Patients in ICU}\tabularnewline 
\midrule\addlinespace[1.5ex]
Reduced Form&&&12.16***&10.75&$-$0.22&4.32&4.45&4.52&0.55&$-$1.58 \tabularnewline
&&&(2.58)&(23.34)&(18.35)&(11.38)&(10.13)&(8.71)&(5.64)&(4.39) \tabularnewline
First stage&&&0.43***&0.33*&0.38***&0.46***&0.45***&0.43***&0.44***&0.41*** \tabularnewline
&&&(0.02)&(0.19)&(0.12)&(0.09)&(0.07)&(0.06)&(0.04)&(0.03) \tabularnewline
> \$10mm funding&41.6***&23.9***&28.37***&24.31&$-$4.01&6.01&1.44&4.36&$-$4.44&$-$11.29 \tabularnewline
&(4.79)&(5.94)&(5.65)&(72.70)&(49.11)&(23.85)&(22.12)&(19.64)&(12.89)&(10.99) \tabularnewline
N&3503&3503&3503&67&181&370&514&671&1321&1868 \tabularnewline
\bottomrule

\end{tabularx}
\caption*{
\scriptsize{\it Notes}: In this table we regress outcomes at the hospital level on a indicator for receiving more than \$10mm in safety net funding. Column 1 presents the results of OLS regression without controls. Column 2 presents the results of OLS controlling for disproportionate patient percentage, uncompensated care per bed, and profit margin.  In columns 3$-$10, we instrument the funding treatment with eligibility to receive this funding and present the results of 2SLS regressions. In columns 3$-$10, the reduced form shows the effect of funding eligibility on the outcome. The first stage shows the effect of funding eligibility on the funding treatment. Column 3 shows the results of a 2SLS regression with no controls.  In columns 4$-$10, we control for the Approximate Propensity Score with different values of bandwidth $\delta$ on the sample with nondegenerate Approximate Propensity Scores. All Approximate Propensity Scores are computed by averaging 10,000 simulation draws. The outcome variables are the 7 day totals for the week spanning July 31st, 2020 to August 6th, 2020. Confirmed COVID patients refer to the sum of patients in inpatient beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Inpatient bed totals also include observation beds. Confirmed COVID patients in ICU refers to the sum of patients in ICU beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Robust standard errors are reported in parentheses. */**/*** indicate p < 0.10/0.05/0.01
}
\label{table:2sls_safetynet_indicator10}
}
\end{table}


==> miscellaneous/tables/Covariate_balance_safety_net_county.tex <==
\newgeometry{left=0.4in, right=0.4in, top=1in}
\begin{table}[h] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Covariate Balance Regressions}
{\scriptsize
\begin{tabularx}{\textwidth}{lCCCCCCCCC}

\toprule
{}&{}&{}&\multicolumn{7}{c}{Our Method: OLS with Approximate Propensity Score Controls} \tabularnewline {}&{Mean}&{No}&\tabularnewline[-2ex] \cline{4-10} \tabularnewline
{}&{(Ineligible Counties)}&{Controls}&{ $\delta = 0.01$}&{ $\delta = 0.025$}&{ $\delta = 0.05$}&{ $\delta = 0.075$}&{ $\delta = 0.1$}&{ $\delta = 0.25$}&{ $\delta = 0.5$} \tabularnewline
&{(1)}&{(2)}&{(3)}&{(4)}&{(5)}&{(6)}&{(7)}&{(8)}&{(9)} \tabularnewline
\midrule\addlinespace[1.5ex]
\tabularnewline[-0.5ex]
\multicolumn{10}{c}{Panel A: Determinants of Funding Eligibility} \\ \tabularnewline[-0.5ex]
Profit margin&.04&$-$0.06***&0.01&$-$0.02&0.02&0.02&0.01&0.01&$-$0.01 \tabularnewline
&&(0.01)&(0.06)&(0.04)&(0.03)&(0.03)&(0.02)&(0.02)&(0.01) \tabularnewline
&&N=2473&N=56&N=151&N=294&N=392&N=524&N=1004&N=1276 \tabularnewline
Uncompensated&58230.92&5,300.32**&5,111.57&5,887.91&$-$4,343.74&$-$9,878.67&$-$7,431.92&$-$2,622.15&939.17 \tabularnewline
care per bed (\$)&&(2,547.93)&(13,153.19)&(11,590.34)&(8,828.13)&(7,834.23)&(6,615.66)&(4,682.76)&(3,163.25) \tabularnewline
&&N=2473&N=56&N=151&N=294&N=392&N=524&N=1004&N=1276 \tabularnewline
Disproportionate&.14&0.19***&0.01&$-$0.07&$-$0.09&$-$0.07&$-$0.08&$-$0.05*&$-$0.03** \tabularnewline
patient percentage&&(0.01)&(0.06)&(0.12)&(0.09)&(0.07)&(0.06)&(0.03)&(0.01) \tabularnewline
&&N=2473&N=56&N=151&N=294&N=392&N=524&N=1004&N=1276 \tabularnewline
\tabularnewline[-0.5ex]
\multicolumn{10}{c}{Panel B: Other Hospital Characteristics} \\ \tabularnewline[-0.5ex]
Full time employees&907.72&4,065.59***&5,666.42*&859.93&$-$690.44&$-$1,240.55&$-$2,168.09***&$-$2,008.24***&$-$2,442.56*** \tabularnewline
&&(457.09)&(3,235.83)&(1,798.20)&(1,248.88)&(938.12)&(803.24)&(444.65)&(316.96) \tabularnewline
&&N=2473&N=56&N=151&N=294&N=392&N=524&N=1004&N=1276 \tabularnewline
Medicare net revenue&17.52&110.34***&138.26**&46.76&$-$9.19&$-$18.16&$-$53.65***&$-$58.07***&$-$65.21*** \tabularnewline
(in millions \$)&&(14.76)&(67.90)&(43.39)&(29.59)&(21.48)&(19.62)&(12.33)&(9.03) \tabularnewline
&&N=2473&N=56&N=151&N=294&N=392&N=524&N=1004&N=1276 \tabularnewline
Occupancy&.38&0.11***&0.20**&0.03&$-$0.04&$-$0.04&$-$0.04&$-$0.02&$-$0.04*** \tabularnewline
&&(0.01)&(0.09)&(0.06)&(0.04)&(0.03)&(0.03)&(0.02)&(0.02) \tabularnewline
&&N=2473&N=56&N=151&N=294&N=392&N=524&N=1004&N=1276 \tabularnewline
Operating margin&0&$-$0.05***&$-$0.01&$-$0.02&0.03&0.02&0.02&0.02&$-$0.00 \tabularnewline
&&(0.01)&(0.06)&(0.04)&(0.03)&(0.03)&(0.02)&(0.02)&(0.01) \tabularnewline
&&N=2473&N=56&N=151&N=294&N=392&N=524&N=1004&N=1276 \tabularnewline
Beds&137.3&586.39***&615.43*&131.88&$-$97.55&$-$172.71&$-$291.81**&$-$319.77***&$-$369.75*** \tabularnewline
&&(64.48)&(346.71)&(241.20)&(190.56)&(145.63)&(118.54)&(66.76)&(45.77) \tabularnewline
&&N=2473&N=56&N=151&N=294&N=392&N=524&N=1004&N=1276 \tabularnewline
Costs per discharge&14.04&2.44&3.50*&3.51**&$-$7.65&1.65&2.88&$-$0.33&0.60 \tabularnewline
(in thousands \$)&&(3.39)&(1.85)&(1.50)&(9.05)&(1.80)&(3.07)&(3.75)&(2.27) \tabularnewline
&&N=2473&N=56&N=151&N=294&N=392&N=524&N=1004&N=1276 \tabularnewline
p-value joint significance&&0&.419&.752&.623&.391&.028&0&0 \tabularnewline
\bottomrule \addlinespace[1.5ex]

\end{tabularx}
\begin{flushleft}
{\it Notes}: This table shows the results of the covariate balance regressions at the county level. The dependent variables for these regressions are drawn from the Healthcare Cost Report Information System for the financial year 2018. Disproportionate patient percentage, profit margin and uncompensated care per bed are used to determine the county's safety net funding eligibility. Other dependent variables shown indicate the financial health and utilization of the counties. In column 2, we regress the dependent variables on the safety net eligibility of the county with no controls. In columns 3–9, we regress the dependent variables on funding eligibility controlling for the Approximate Propensity Score with different values of bandwidth $\delta$. All Approximate Propensity Scores are computed by averaging 10,000 simulation draws. Column 1 shows the mean of dependent variables for counties that are ineligible to receive safety net funding. Robust standard errors are reported in the parenthesis and the number of observations is reported separately for each regression. The last row reports the p-value of the joint significance test. */**/*** indicate $p <$ 0.10/0.05/0.01
\end{flushleft}
}
\label{table:CBR_C}
\end{table}
\restoregeometry


==> miscellaneous/tables/Covariate_balance_safety_net_county_s.tex <==
\newgeometry{margin=0.15in}
\begin{table}[h] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Covariate Balance Regressions}
{\scriptsize
\begin{tabularx}{\textwidth}{lCCCCCCCCC}

\toprule
&{(1)}&{(2)}&{(3)}&{(4)}&{(5)}&{(6)}&{(7)}&{(8)}&{(9)} \tabularnewline
{}&{}&{}&\multicolumn{7}{c}{Our Method: OLS with Approximate Propensity Score Controls} \tabularnewline {}&{Mean}&{No}&\tabularnewline[-2ex] \cline{4-10} \tabularnewline
{}&{(Ineligible Counties)}&{Controls}&{ $\delta = 0.005$}&{ $\delta = 0.01$}&{ $\delta = 0.015$}&{ $\delta = 0.02$}&{ $\delta = 0.03$}&{ $\delta = 0.04$}&{ $\delta = 0.05$} \tabularnewline
\midrule\addlinespace[1.5ex]
Profit margin&.04&$-$0.06***&$-$0.04&0.01&0.01&$-$0.02&0.02&0.04&0.03 \tabularnewline
&&(0.01)&(0.09)&(0.06)&(0.05)&(0.05)&(0.03)&(0.03)&(0.03) \tabularnewline
&&N=2473&N=24&N=56&N=79&N=121&N=178&N=231&N=294 \tabularnewline
Uncompensated&58230.92&5,300.32**&13,484.74&5,529.70&9,562.34&15,209.48&267.63&544.28&$-$4,319.30 \tabularnewline
care per bed (\$)&&(2,547.93)&(15,647.02)&(13,369.45)&(12,622.40)&(13,018.14)&(12,052.66)&(10,474.49)&(9,086.00) \tabularnewline
&&N=2473&N=24&N=56&N=79&N=121&N=178&N=231&N=294 \tabularnewline
Disproportionate&.14&0.19***&$-$0.09&0.00&0.06&$-$0.07&$-$0.09&$-$0.08&$-$0.08 \tabularnewline
patient percentage&&(0.01)&(0.07)&(0.06)&(0.08)&(0.10)&(0.11)&(0.10)&(0.09) \tabularnewline
&&N=2473&N=24&N=56&N=79&N=121&N=178&N=231&N=294 \tabularnewline
Full time employees&907.72&4,065.59***&4,626.82&5,605.38*&3,141.61&2,014.46&846.19&148.36&$-$661.24 \tabularnewline
&&(457.09)&(3,344.42)&(3,256.64)&(2,504.61)&(2,093.97)&(1,638.31)&(1,433.35)&(1,263.80) \tabularnewline
&&N=2473&N=24&N=56&N=79&N=121&N=178&N=231&N=294 \tabularnewline
Medicare net revenue&17.52&110.34***&73.27&134.81*&91.08*&65.27&37.24&11.92&$-$8.85 \tabularnewline
(in millions \$)&&(14.76)&(60.08)&(68.54)&(52.82)&(49.54)&(38.96)&(33.09)&(29.63) \tabularnewline
&&N=2473&N=24&N=56&N=79&N=121&N=178&N=231&N=294 \tabularnewline
Occupancy&.38&0.11***&0.13&0.20**&0.09&0.09&0.03&$-$0.01&$-$0.03 \tabularnewline
&&(0.01)&(0.13)&(0.09)&(0.07)&(0.07)&(0.06)&(0.05)&(0.04) \tabularnewline
&&N=2473&N=24&N=56&N=79&N=121&N=178&N=231&N=294 \tabularnewline
Operating margin&0&$-$0.05***&$-$0.05&$-$0.00&0.01&$-$0.03&0.02&0.04&0.03 \tabularnewline
&&(0.01)&(0.09)&(0.06)&(0.05)&(0.06)&(0.03)&(0.03)&(0.03) \tabularnewline
&&N=2473&N=24&N=56&N=79&N=121&N=178&N=231&N=294 \tabularnewline
Beds&137.3&586.39***&588.70&597.23*&388.49&298.20&107.78&7.15&$-$93.82 \tabularnewline
&&(64.48)&(418.25)&(353.44)&(280.73)&(271.99)&(226.70)&(212.24)&(191.39) \tabularnewline
&&N=2473&N=24&N=56&N=79&N=121&N=178&N=231&N=294 \tabularnewline
Costs per discharge&14.04&2.44&3.99**&3.42*&3.92**&2.34&2.86**&1.97*&$-$7.56 \tabularnewline
(in thousands \$)&&(3.39)&(1.86)&(1.90)&(1.58)&(1.49)&(1.27)&(1.12)&(9.00) \tabularnewline
&&N=2473&N=24&N=56&N=79&N=121&N=178&N=231&N=294 \tabularnewline
p-value joint significance&&0&.723&.45&.763&.856&.791&.755&.626 \tabularnewline
\bottomrule \addlinespace[1.5ex]

\end{tabularx}
\begin{flushleft}
\footnotesize {\it Notes}: This table shows the results of the covariate balance regressions at the county level. The dependent variables for these regressions are drawn from the Healthcare Cost Report Information System for the financial year 2018. Disproportionate patient percentage, profit margin and uncompensated care per bed are used to determine the county's safety net funding eligibility. Other dependent variables shown indicate the financial health and utilization of the counties. In column 2, we regress the dependent variables on the safety net eligibility of the county with no controls. In columns 3–9, we regress the dependent variables on funding eligibility controlling for the Approximate Propensity Score with different values of bandwidth $\delta$. All Approximate Propensity Scores are computed by averaging 10,000 simulation draws. Column 1 shows the mean of dependent variables for counties that are ineligible to receive safety net funding. Robust standard errors are reported in the parenthesis and the number of observations is reported separately for each regression. The last row reports the p-value of the joint significance test. */**/*** indicate p < 0.10/0.05/0.01
\end{flushleft}
}
\end{table}
\restoregeometry


==> miscellaneous/tables/Covariate_balance_safety_net_dist.tex <==
\newgeometry{margin=0.15in}
\begin{table}[h] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Covariate Balance Regressions}
{\scriptsize
\begin{tabularx}{\textwidth}{lCCCCCCCCCC}

\toprule
{}&{}&{}&\multicolumn{8}{c}{RD with Linear Boundary Distance Controls} \tabularnewline {}&{Mean}&{No}&\tabularnewline[-2ex] \cline{4-11} \tabularnewline
{}&{(Ineligible Hospitals)}&{Controls}&{ $\delta = 0.01$}&{ $\delta = 0.025$}&{ $\delta = 0.05$}&{ $\delta = 0.075$}&{ $\delta = 0.1$}&{ $\delta = 0.25$}&{ $\delta = CCT$}&{ $\delta = IK$} \tabularnewline
&{(1)}&{(2)}&{(3)}&{(4)}&{(5)}&{(6)}&{(7)}&{(8)}&{(9)}&{(10)} \tabularnewline
\midrule\addlinespace[1.5ex]
\tabularnewline[-0.5ex]
\multicolumn{10}{c}{Panel A: Determinants of Funding Eligibility} \\ \tabularnewline[-0.5ex]
Profit margin&.04&-0.11***&-0.02&-0.01&0.00&-0.01&0.00&0.02&0.02*&0.03** \tabularnewline
&&(0.01)&(0.05)&(0.04)&(0.03)&(0.03)&(0.02)&(0.01)&(0.01)&(0.01) \tabularnewline
&&N=4633&N=91&N=239&N=487&N=677&N=890&N=1734&N=1892&N=2005 \tabularnewline
Uncompensated&56556.02&19,540.28***&2,259.99&8,593.97&-1,323.32&-3,960.02&-130.93&5,816.54&206.46&8,978.81** \tabularnewline
care per bed (\$)&&(3,827.22)&(10,099.31)&(9,756.36)&(8,368.94)&(7,327.22)&(6,881.87)&(4,427.05)&(5,215.59)&(4,087.85) \tabularnewline
&&N=4633&N=91&N=239&N=487&N=677&N=890&N=1734&N=1321&N=1919 \tabularnewline
Disproportionate&.18&0.21***&-0.05&-0.08&-0.07&-0.05&-0.05&-0.02&-0.02&-0.01 \tabularnewline
patient percentage&&(0.01)&(0.07)&(0.07)&(0.06)&(0.05)&(0.04)&(0.02)&(0.02)&(0.01) \tabularnewline
&&N=4633&N=91&N=239&N=487&N=677&N=890&N=1734&N=1834&N=2291 \tabularnewline
\tabularnewline[-0.5ex]
\multicolumn{10}{c}{Panel B: Other Hospital Characteristics} \\ \tabularnewline[-0.5ex]
Full time employees&897.32&454.26***&1,994.72&310.75&18.05&148.02&83.30&179.95&242.17&217.58 \tabularnewline
&&(69.23)&(1,535.08)&(916.47)&(558.94)&(428.44)&(346.31)&(197.09)&(171.24)&(164.87) \tabularnewline
&&N=4626&N=91&N=238&N=486&N=676&N=889&N=1731&N=2039&N=2103 \tabularnewline
Medicare net revenue&20.04&18.36***&24.59&-6.84&-1.24&4.27&7.83&6.55&9.38&9.12* \tabularnewline
(in millions \$)&&(2.39)&(26.57)&(17.15)&(13.18)&(11.20)&(9.96)&(6.17)&(5.87)&(5.51) \tabularnewline
&&N=4511&N=90&N=238&N=485&N=673&N=886&N=1692&N=1812&N=2001 \tabularnewline
Occupancy&.44&0.07***&0.15*&0.05&-0.01&0.01&0.01&0.03*&0.03*&0.02 \tabularnewline
&&(0.01)&(0.08)&(0.05)&(0.04)&(0.03)&(0.03)&(0.02)&(0.02)&(0.02) \tabularnewline
&&N=4624&N=91&N=239&N=487&N=677&N=890&N=1734&N=1729&N=1692 \tabularnewline
Operating margin&.02&-0.11***&-0.02&-0.01&0.00&-0.00&0.02&0.03*&0.03**&0.03** \tabularnewline
&&(0.01)&(0.05)&(0.04)&(0.03)&(0.03)&(0.02)&(0.02)&(0.01)&(0.01) \tabularnewline
&&N=4541&N=90&N=238&N=479&N=667&N=879&N=1684&N=1877&N=2038 \tabularnewline
Beds&134.6&53.75***&150.26&23.13&-0.48&12.33&14.10&11.65&24.70&16.82 \tabularnewline
&&(7.05)&(97.01)&(60.92)&(41.67)&(33.77)&(28.37)&(17.82)&(15.98)&(14.57) \tabularnewline
&&N=4633&N=91&N=239&N=487&N=677&N=890&N=1734&N=1983&N=2201 \tabularnewline
Costs per discharge&66.28&-49.95***&3.99**&2.92**&1.41&-6.73&1.51*&5.58&3.18&5.42 \tabularnewline
(in thousands \$)&&(17.93)&(1.90)&(1.43)&(1.12)&(8.61)&(0.88)&(4.50)&(2.43)&(3.98) \tabularnewline
&&N=3539&N=91&N=239&N=487&N=677&N=890&N=1734&N=1038&N=1274 \tabularnewline
p-value joint significance&&0&.716&.513&.97&.966&.701&.111&.&. \tabularnewline
\bottomrule \addlinespace[1.5ex]

\end{tabularx}
\begin{flushleft}
{\it Notes}: This table shows the results of the covariate balance regressions at the hospital level. The dependent variables for these regressions are drawn from the Healthcare Cost Report Information System for the financial year 2018. Disproportionate patient percentage, profit margin and uncompensated care per bed are used to determine the hospital's safety net funding eligibility. Other dependent variables shown indicate the financial health and utilization of the hospitals. In column 2, we regress the dependent variables on the safety net eligibility of the hospital with no controls. In columns 3–10, we regress the dependent variables on funding eligibility linearly controlling for the boundary distance and using different values of bandwidth $\delta$. Column 9 uses the Calonico, Cattaneo and Titiunik (2014) optimal MSE bandwidth computed separately for each dependent variable. Column 10 uses the Imbens and Kalyanaraman (2012) optimal MSE bandwidth computed separately for each dependent variable. Column 1 shows the mean of dependent variables for hospitals that are ineligible to receive safety net funding. Robust standard errors are reported in the parenthesis and the number of observations is reported separately for each regression. The last row reports the p-value of the joint significance test.  */**/*** indicate p < 0.10/0.05/0.01
\end{flushleft}
}
\end{table}
\restoregeometry


==> miscellaneous/tables/Covariate_balance_safety_net_mid.tex <==
\newgeometry{margin=0.15in}
\begin{table}[h] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Covariate Balance Regressions}
{\tiny
\begin{tabularx}{\textwidth}{lCCCCCCCCC}

\toprule
&{(1)}&{(2)}&{(3)}&{(4)}&{(5)}&{(6)}&{(7)}&{(8)}&{(9)} \tabularnewline
{}&{}&{}&\multicolumn{7}{c}{Our Method: OLS with Approximate Propensity Score Controls} \tabularnewline {}&{Mean}&{No}&\tabularnewline[-2ex] \cline{4-10} \tabularnewline
{}&{(Ineligible Hospitals)}&{Controls}&{ $\delta = 0.01$}&{ $\delta = 0.025$}&{ $\delta = 0.05$}&{ $\delta = 0.075$}&{ $\delta = 0.1$}&{ $\delta = 0.25$}&{ $\delta = 0.5$} \tabularnewline
\midrule\addlinespace[1.5ex]
Profit margin&.04&-0.10***&-0.03&0.01&0.04&0.01&0.03&0.07***&0.08*** \tabularnewline
&&(0.01)&(0.06)&(0.05)&(0.03)&(0.03)&(0.03)&(0.02)&(0.01) \tabularnewline
&&N=4300&N=65&N=184&N=382&N=541&N=724&N=1452&N=2051 \tabularnewline
Uncompensated&56556.02&17,940.20***&12,356.10&10,238.58&-11,586.97&-18,076.40**&-17,058.00***&-8,239.15&-4,707.65 \tabularnewline
care per bed (\$)&&(4,756.10)&(12,288.91)&(9,693.95)&(7,182.81)&(7,129.04)&(6,571.11)&(5,100.88)&(4,323.28) \tabularnewline
&&N=4300&N=65&N=184&N=382&N=541&N=724&N=1452&N=2051 \tabularnewline
Disproportionate&.18&0.23***&-0.10&-0.09&-0.09&-0.08&-0.08&-0.05*&-0.06*** \tabularnewline
patient percentage&&(0.01)&(0.10)&(0.08)&(0.09)&(0.07)&(0.06)&(0.03)&(0.02) \tabularnewline
&&N=4300&N=65&N=184&N=382&N=541&N=724&N=1452&N=2051 \tabularnewline
Full time employees&897.32&773.91***&1,960.33&238.74&8.44&101.46&231.27&489.70**&457.49*** \tabularnewline
&&(72.94)&(1,176.66)&(853.55)&(680.33)&(535.04)&(441.52)&(239.31)&(156.89) \tabularnewline
&&N=4294&N=65&N=184&N=382&N=541&N=724&N=1450&N=2049 \tabularnewline
Medicare net revenue&20.04&27.09***&26.48&-2.18&-5.79&-4.79&3.11&6.90&5.13 \tabularnewline
(in millions \$)&&(2.67)&(26.94)&(17.12)&(15.26)&(12.53)&(11.41)&(6.94)&(4.98) \tabularnewline
&&N=4178&N=64&N=183&N=380&N=537&N=720&N=1410&N=2006 \tabularnewline
Occupancy&.44&0.15***&0.21**&0.11*&0.05&0.06*&0.08**&0.11***&0.14*** \tabularnewline
&&(0.01)&(0.11)&(0.07)&(0.05)&(0.04)&(0.03)&(0.02)&(0.02) \tabularnewline
&&N=4291&N=65&N=184&N=382&N=541&N=724&N=1452&N=2051 \tabularnewline
Operating margin&.02&-0.10***&-0.03&0.02&0.04&0.02&0.04&0.08***&0.10*** \tabularnewline
&&(0.01)&(0.06)&(0.05)&(0.04)&(0.04)&(0.03)&(0.02)&(0.02) \tabularnewline
&&N=4209&N=65&N=184&N=375&N=532&N=714&N=1403&N=1998 \tabularnewline
Beds&134.6&109.32***&188.15*&85.56&44.01&47.20&64.38*&70.24***&69.06*** \tabularnewline
&&(7.46)&(105.41)&(68.13)&(51.88)&(42.55)&(35.92)&(21.72)&(15.63) \tabularnewline
&&N=4300&N=65&N=184&N=382&N=541&N=724&N=1452&N=2051 \tabularnewline
Costs per discharge&66.28&-52.51***&5.14*&5.32***&2.77**&2.20*&1.93**&1.80**&6.67 \tabularnewline
(in thousands \$)&&(17.79)&(2.61)&(1.65)&(1.26)&(1.12)&(0.93)&(0.76)&(6.62) \tabularnewline
&&N=3206&N=65&N=184&N=382&N=541&N=724&N=1452&N=2051 \tabularnewline
p-value joint significance&&0&.45&.021&.092&.008&.001&0&0 \tabularnewline
\bottomrule \addlinespace[1.5ex]

\end{tabularx}
\begin{flushleft}
\tiny {\it Notes}: This table shows the results of the covariate balance regressions at the hospital level. The dependent variables for these regressions are drawn from the Healthcare Cost Report Information System for the financial year 2018. Disproportionate patient percentage, profit margin and uncompensated care per bed are used to determine the hospital's safety net funding eligibility. Other dependent variables shown indicate the financial health and utilization of the hospitals. In column 2, we regress the dependent variables on the safety net eligibility of the hospital with no controls. In columns 3–9, we regress the dependent variables on funding eligibility controlling for the Approximate Propensity Score with different values of bandwidth $\delta$. All Approximate Propensity Scores are computed by averaging 10,000 simulation draws. Column 1 shows the mean of dependent variables for hospitals that are ineligible to receive safety net funding. Robust standard errors are reported in the parenthesis and the number of observations is reported separately for each regression. The last row reports the p-value of the joint significance test. */**/*** indicate p < 0.10/0.05/0.01
\end{flushleft}
}
\end{table}
\restoregeometry


==> miscellaneous/tables/reduced_form_safety_net.tex <==
\newgeometry{margin=0.15in}
\begin{table}[h] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Effects of Funding Eligibility on Hospital Behavior}
{\tiny
\begin{tabularx}{\linewidth}{lCCCCCCCCC}

\toprule
&{(1)}&{(2)}&{(3)}&{(4)}&{(5)}&{(6)}&{(7)}&{(8)}&{(9)} \tabularnewline \midrule
{}&{}&{}&\multicolumn{7}{c}{Our Method: OLS with Approximate Propensity Score Controls} \tabularnewline {}&{Mean}&{OLS}&\tabularnewline[-2ex] \cline{4-10} \tabularnewline
{}&{}&{No Controls}&{ $\delta = 0.01$}&{ $\delta = 0.025$}&{ $\delta = 0.05$}&{ $\delta = 0.075$}&{ $\delta = 0.1$}&{ $\delta = 0.25$}&{ $\delta = 0.5$} \tabularnewline
\midrule \addlinespace[\belowrulesep]
\# Confirmed COVID Patients&105.6&33.97***&8.82&$-$31.57&25.21&15.28&10.63&9.17&5.23 \tabularnewline
&&(7.44)&(66.76)&(54.25)&(34.19)&(30.38)&(25.91)&(15.96)&(12.41) \tabularnewline
&&N=3558&N=70&N=191&N=385&N=539&N=709&N=1366&N=1923 \tabularnewline
\# Confirmed COVID Patients in ICU&80.1&12.16***&10.75&$-$0.22&4.32&4.45&4.52&0.55&$-$1.58 \tabularnewline
&&(2.58)&(23.34)&(18.35)&(11.38)&(10.13)&(8.71)&(5.64)&(4.39) \tabularnewline
&&N=3503&N=67&N=181&N=370&N=514&N=671&N=1321&N=1868 \tabularnewline
\# Confirmed/Suspected COVID Patients&31.38&38.19***&8.41&$-$20.86&$-$40.66&$-$44.36&$-$28.22&15.52&12.52 \tabularnewline
&&(8.55)&(73.91)&(69.28)&(75.21)&(67.30)&(51.72)&(23.22)&(15.80) \tabularnewline
&&N=3532&N=73&N=195&N=392&N=547&N=719&N=1389&N=1947 \tabularnewline
\# Confirmed/Suspected COVID Patients in ICU&26.62&13.18***&16.80&10.38&6.89&2.94&5.05&2.25&$-$0.24 \tabularnewline
&&(2.74)&(21.19)&(17.28)&(12.12)&(10.88)&(9.21)&(5.83)&(4.62) \tabularnewline
&&N=3445&N=72&N=186&N=374&N=520&N=678&N=1314&N=1846 \tabularnewline
&&&&&&&&& \tabularnewline
\bottomrule \addlinespace[\belowrulesep]

\end{tabularx}
\begin{flushleft}
\tiny {\it Notes}: This table shows the results of reduced form regressions of hospital level outcomes on an indicator for being eligible for safety net funding. Column 1 shows the mean of dependent variables for hospitals. In column 2, we regress the dependent variables on the safety net eligibility of the hospital. In columns 3–9, we regress the dependent variables on funding eligibility controlling for the Approximate Propensity Score with different values of bandwidth $\delta$. We also control for disproportionate patient percentage, uncompensated care per bed, and profit margin in columns 3–9. All Approximate Propensity Scores are computed by averaging 10,000 simulation draws. The outcome variables are the 7 day totals for the week spanning July 31st, 2020 to August 6th, 2020. Confirmed or Suspected COVID patients refer to the sum of patients in inpatient beds with lab-confirmed/suspected COVID-19. Confirmed COVID patients refer to the sum of patients in inpatient beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Inpatient bed totals also include observation beds. Similarly, Confirmed/Suspected COVID patients in ICU refer to the sum of patients in ICU beds with lab-confirmed or suspected COVID-19. Confirmed COVID patients in ICU refers to the sum of patients in ICU beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Robust standard errors are reported in the parentheses and the number of observations is reported separately for each regression. The last row reports the p-value of the joint significance test. */**/*** indicate p < 0.10/0.05/0.01
\end{flushleft}
}
\end{table}
\restoregeometry


==> miscellaneous/tables/z_aps.tex <==
\begin{table}[h] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Dependent Variable: Funding Eligibility Dummy}
{\scriptsize
\begin{tabularx}{\textwidth}{lCCCCCCCC}

\toprule
{}&{$\delta = $}&{$\delta = $}&{$\delta = $}&{$\delta = $}&{$\delta = $}&{$\delta = $}&{$\delta = $}&{$\delta = $} \tabularnewline
{}&{0.005}&{0.01}&{0.025}&{0.05}&{0.075}&{0.1}&{0.25}&{0.5} \tabularnewline
\midrule\addlinespace[1.5ex]
APS&1.31&1.26&1.27&1.27&1.31&1.29&1.35&1.50 \tabularnewline
&(0.05)&(0.03)&(0.02)&(0.02)&(0.01)&(0.01)&(0.01)&(0.02) \tabularnewline
N&39&89&239&485&671&879&1726&2368 \tabularnewline
\bottomrule \addlinespace[1.5ex]

\end{tabularx}
\begin{flushleft}
\scriptsize {\it Notes}: In this table we regress an indicator for receiving safety net funding on Approximate Propensity Scores with different values of bandwidth $\delta$ on the sample with nondegenerate Approximate Propensity Scores. All Approximate Propensity Scores are computed by averaging 10,000 simulation draws. Robust standard errors are reported in parentheses.
\end{flushleft}
}
\end{table}


==> miscellaneous/tables/z_aps_full.tex <==
\begin{table}[h] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Dependent Variable: Funding Eligibility Dummy}
{\scriptsize
\begin{tabularx}{\textwidth}{lCCCCCCCC}

\toprule
{}&{$\delta = $}&{$\delta = $}&{$\delta = $}&{$\delta = $}&{$\delta = $}&{$\delta = $}&{$\delta = $}&{$\delta = $} \tabularnewline
{}&{0.005}&{0.01}&{0.025}&{0.05}&{0.075}&{0.1}&{0.25}&{0.5} \tabularnewline
\midrule\addlinespace[1.5ex]
APS&1.00&1.00&1.01&1.03&1.04&1.05&1.14&1.29 \tabularnewline
&(0.00)&(0.00)&(0.00)&(0.00)&(0.00)&(0.00)&(0.01)&(0.01) \tabularnewline
N&4633&4633&4633&4633&4633&4633&4633&4633 \tabularnewline
\bottomrule \addlinespace[1.5ex]

\end{tabularx}
\begin{flushleft}
\scriptsize {\it Notes}: In this table we regress an indicator for receiving safety net funding on Approximate Propensity Scores with different values of bandwidth $\delta$ on the full sample. All Approximate Propensity Scores are computed by averaging 10,000 simulation draws. Robust standard errors are reported in parentheses.
\end{flushleft}
}
\end{table}


==> tables/2SLS_safety_net_combined.tex <==
\begin{table}[!t] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Effects of Funding on Hospital Behavior}
{\scriptsize
\begin{tabularx}{\textwidth}{lCCCCCCCCCC}

\hline\tabularnewline[-1.8ex]
{}&{OLS with}&{OLS with}&{2SLS with}&\multicolumn{7}{c}{Our Method: 2SLS with Approximate Propensity Score Controls} \tabularnewline
{}&{No}&{Covariate}&{No} \tabularnewline[-1.8ex]\cline{5-11} \tabularnewline[-1.8ex]
{}&{Controls}&{Controls}&{Controls}&{ $\delta = 0.01$}&{ $\delta = 0.025$}&{ $\delta = 0.05$}&{ $\delta = 0.075$}&{ $\delta = 0.1$}&{ $\delta = 0.25$}&{ $\delta = 0.5$} \tabularnewline
&(1)&(2)&(3)&(4)&(5)&(6)&(7)&(8)&(9)&(10)\\
\midrule\addlinespace[1.5ex]
\multicolumn{11}{l}{\# Confirmed COVID Patients:}\tabularnewline
\addlinespace[0.75ex]
~~First stage&&&13.90&15.85&14.26&14.68&14.47&14.19&13.82&12.77 \tabularnewline
~~(in millions \$)&&&(0.50)&(5.49)&(3.17)&(2.02)&(1.62)&(1.40)&(0.90)&(0.66) \tabularnewline
~~Reduced form&&&33.97&$-$7.51&$-$31.50&15.98&0.47&0.54&$-$7.80&$-$19.45 \tabularnewline
&&&(7.44)&(71.05)&(48.48)&(29.66)&(25.39)&(20.88)&(13.73)&(12.61) \tabularnewline
~~\$1mm of funding&4.53&2.50&2.44&$-$0.47&$-$2.21&1.09&0.03&0.04&$-$0.56&$-$1.52  \tabularnewline
&(0.63)&(0.79)&(0.50)&(4.42)&(3.53)&(1.97)&(1.75)&(1.47)&(1.01)&(1.01) \tabularnewline
~~N&3558&3558&3558&72&191&393&550&725&1388&1949 \tabularnewline
\addlinespace[1.5ex]
\multicolumn{10}{l}{\# Confirmed COVID Patients in ICU:}\tabularnewline
\addlinespace[0.75ex]
~~First stage&&&13.89&15.03&13.99&15.61&15.12&14.77&14.07&12.92 \tabularnewline
~~(in millions \$)&&&(0.50)&(5.62)&(3.19)&(2.08)&(1.71)&(1.47)&(0.94)&(0.68) \tabularnewline
~~Reduced form&&&12.16&4.42&$-$1.71&2.05&0.54&1.61&$-$4.21&$-$7.82 \tabularnewline
&&&(2.58)&(24.19)&(16.89)&(9.89)&(8.52)&(7.17)&(4.87)&(4.34) \tabularnewline
~~\$1mm of funding&1.51&0.82&0.88&0.29&$-$0.12&0.13&0.04&0.11&$-$0.30&$-$0.61 \tabularnewline
&(0.21)&(0.27)&(0.17)&(1.56)&(1.20)&(0.63)&(0.56)&(0.48)&(0.35)&(0.35) \tabularnewline
~~N&3503&3503&3503&68&181&379&526&689&1342&1893 \tabularnewline
\bottomrule %\addlinespace[1.5ex]

\end{tabularx}
\caption*{
\scriptsize{\it Note}: In this table, we estimate the effects of the funding amount on hospital-level outcomes. Column 1 presents OLS results of outcome variables on funding without controls. Column 2 controls for disproportionate patient percentage, uncompensated care per bed, and profit margin. Column 3 shows the results of 2SLS regression with no controls. In columns 4--10, we control for Approximate Propensity Score with different values of bandwidth $\delta$ on the sample with nondegenerate Approximate Propensity Scores. The first stage shows the effect of funding eligibility on the amount of relief funding received by hospitals, in millions of dollars. The reduced form shows the effect of funding eligibility on the outcome. 2SLS estimates show the effect of the amount of relief funding on outcomes. Approximate Propensity Scores are computed by averaging 10,000 simulation draws. The outcome variables are 7 day totals for the week spanning July 31st, 2020 to August 6th, 2020. Confirmed COVID patients refer to the sum of patients in inpatient beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Inpatient bed totals also include observation beds. Confirmed COVID patients in ICU refers to the sum of patients in ICU beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Robust standard errors are reported in parentheses.
}
\label{table:2sls_safetynet}
}
\end{table}


==> tables/deprecated/2SLS_safety_net.tex <==
\begin{table}[!t] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Effects of Funding on Hospital Behavior: Funding Amount Treatment}
{\scriptsize
\begin{tabularx}{\textwidth}{lCCCCCCCCCC}

\hline\hline\tabularnewline[-1.8ex]
{}&{OLS with}&{OLS with}&{2SLS with}&\multicolumn{7}{c}{Our Method: 2SLS with Approximate Propensity Score Controls} \tabularnewline
{}&{No}&{Covariate}&{No} \tabularnewline[-1.8ex]\cline{5-11} \tabularnewline[-1.8ex]
{}&{Controls}&{Controls}&{Controls}&{ $\delta = 0.01$}&{ $\delta = 0.025$}&{ $\delta = 0.05$}&{ $\delta = 0.075$}&{ $\delta = 0.1$}&{ $\delta = 0.25$}&{ $\delta = 0.5$} \tabularnewline
&(1)&(2)&(3)&(4)&(5)&(6)&(7)&(8)&(9)&(10)\\
\midrule\addlinespace[1.5ex]
\multicolumn{11}{l}{\# Confirmed/Suspected COVID Patients}\tabularnewline
\midrule\addlinespace[1.5ex]
First stage&&&13.78***&15.11**&13.34***&14.28***&14.19***&13.89***&13.96***&13.06*** \tabularnewline
(in millions \$)&&&(0.49)&(5.83)&(3.54)&(2.27)&(1.87)&(1.61)&(1.03)&(0.74) \tabularnewline
\$1mm of funding&5.58***&3.25***&2.77***&$-$1.03&$-$1.86&$-$3.10&$-$4.08&$-$2.91&0.15&$-$0.31 \tabularnewline
&(0.68)&(0.89)&(0.58)&(5.64)&(5.40)&(4.99)&(4.57)&(3.58)&(1.59)&(1.21) \tabularnewline
N&3532&3532&3532&73&195&392&547&719&1389&1947 \tabularnewline
\midrule\addlinespace[1.5ex]
\multicolumn{11}{l}{\# Confirmed COVID Patients}\tabularnewline
\midrule\addlinespace[1.5ex]
First stage&&&13.90***&16.55***&14.37***&15.05***&14.81***&14.42***&14.10***&13.19*** \tabularnewline
(in millions \$)&&&(0.50)&(6.11)&(3.66)&(2.33)&(1.91)&(1.64)&(1.04)&(0.75) \tabularnewline
\$1mm of funding&4.53***&2.50***&2.44***&0.05&$-$2.14&1.42&0.13&$-$0.03&$-$0.09&$-$0.63 \tabularnewline
&(0.63)&(0.79)&(0.50)&(4.33)&(3.97)&(2.17)&(1.97)&(1.74)&(1.12)&(0.96) \tabularnewline
N&3558&3558&3558&70&191&385&539&709&1366&1923 \tabularnewline
\midrule\addlinespace[1.5ex]
\multicolumn{10}{l}{\# Confirmed/Suspected COVID Patients in ICU}\tabularnewline 
\midrule\addlinespace[1.5ex]
First stage&&&13.88***&14.67**&13.42***&15.75***&15.29***&14.74***&14.31***&13.18*** \tabularnewline
(in millions \$)&&&(0.51)&(5.59)&(3.49)&(2.32)&(1.93)&(1.67)&(1.06)&(0.76) \tabularnewline
\$1mm of funding&1.67***&0.91***&0.95***&0.93&0.71&0.36&$-$0.05&0.16&$-$0.03&$-$0.32 \tabularnewline
&(0.21)&(0.28)&(0.18)&(1.47)&(1.27)&(0.74)&(0.70)&(0.60)&(0.40)&(0.36) \tabularnewline
N&3445&3445&3445&72&186&374&520&678&1314&1846 \tabularnewline
\midrule\addlinespace[1.5ex]
\multicolumn{10}{l}{\# Confirmed COVID Patients in ICU}\tabularnewline
\midrule\addlinespace[1.5ex]
First stage&&&13.89***&15.80**&13.79***&15.78***&15.53***&15.08***&14.43***&13.40*** \tabularnewline
(in millions \$)&&&(0.50)&(6.15)&(3.73)&(2.41)&(2.02)&(1.73)&(1.09)&(0.77) \tabularnewline
\$1mm of funding&1.51***&0.82***&0.88***&0.50&$-$0.11&0.18&0.04&0.12&$-$0.13&$-$0.35 \tabularnewline
&(0.21)&(0.27)&(0.17)&(1.54)&(1.37)&(0.70)&(0.64)&(0.56)&(0.39)&(0.34) \tabularnewline
N&3503&3503&3503&67&181&370&514&671&1321&1868 \tabularnewline
\bottomrule %\addlinespace[1.5ex]

\end{tabularx}
\caption*{
\scriptsize{\it Notes}: In this table we regress relevant outcomes at the hospital level on the amount of funding. Column 1 presents the results of OLS regression of the outcome variables on funding without any controls. Column 2 presents the results of OLS regression of the outcome variables on funding controlling for disproportionate patient percentage, uncompensated care per bed and profit margin.  In columns 3--10, we instrument the amount of funding with eligibility to receive this funding and present the results of 2SLS regressions. In columns 3--10, the first stage shows the effect of being deemed eligible on the amount of relief funding received by hospitals, in millions of dollars. Column 3 shows the results of a 2SLS regression with no controls.  In columns 4--10, we run this regression controlling for the Approximate Propensity Score with different values of bandwidth $\delta$ on the sample with nondegenerate Approximate Propensity Scores.  All Approximate Propensity Scores are computed by averaging 10,000 simulation draws. The outcome variables are the 7 day totals for the week spanning July 31st, 2020 to August 6th, 2020. Confirmed or Suspected COVID patients refer to the sum of patients in inpatient beds with lab-confirmed/suspected COVID-19. Confirmed COVID patients refer to the sum of patients in inpatient beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Inpatient bed totals also include observation beds. Similarly, Confirmed/Suspected COVID patients in ICU refer to the sum of patients in ICU beds with lab-confirmed or suspected COVID-19. Confirmed COVID patients in ICU refers to the sum of patients in ICU beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Robust standard errors are reported in parentheses. */**/*** indicate $p <$ 0.10/0.05/0.01.
}
\label{table:2sls_safetynet}
}
\end{table}
%\restoregeometry

==> tables/deprecated/2SLS_safety_net_combined.tex <==
\begin{table}[!t] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Effects of Funding on Hospital Behavior}
{\scriptsize
\begin{tabularx}{\textwidth}{lCCCCCCCCCC}

\hline\tabularnewline[-1.8ex]
{}&{OLS with}&{OLS with}&{2SLS with}&\multicolumn{7}{c}{Our Method: 2SLS with Approximate Propensity Score Controls} \tabularnewline
{}&{No}&{Covariate}&{No} \tabularnewline[-1.8ex]\cline{5-11} \tabularnewline[-1.8ex]
{}&{Controls}&{Controls}&{Controls}&{ $\delta = 0.01$}&{ $\delta = 0.025$}&{ $\delta = 0.05$}&{ $\delta = 0.075$}&{ $\delta = 0.1$}&{ $\delta = 0.25$}&{ $\delta = 0.5$} \tabularnewline
&(1)&(2)&(3)&(4)&(5)&(6)&(7)&(8)&(9)&(10)\\
\midrule\addlinespace[1.5ex]
\multicolumn{11}{l}{\# Confirmed COVID Patients:}\tabularnewline
\addlinespace[0.75ex]
~~First stage&&&13.90&16.55&14.37&15.05&14.81&14.42&14.10&13.19 \tabularnewline
~~(in millions \$)&&&(0.50)&(6.11)&(3.66)&(2.33)&(1.91)&(1.64)&(1.04)&(0.75) \tabularnewline
~~Reduced form&&&33.97&8.82&$-$31.57&25.21&15.28&10.63&9.17&5.23 \tabularnewline
&&&(7.44)&(66.76)&(54.25)&(34.19)&(30.38)&(25.91)&(15.96)&(12.41) \tabularnewline
~~\$1mm of funding&4.53&2.50&2.44&0.05&$-$2.14&1.42&0.13&$-$0.03&$-$0.09&$-$0.63 \tabularnewline
&(0.63)&(0.79)&(0.50)&(4.33)&(3.97)&(2.17)&(1.97)&(1.74)&(1.12)&(0.96) \tabularnewline
~~N&3558&3558&3558&70&191&385&539&709&1366&1923 \tabularnewline
\addlinespace[1.5ex]
\multicolumn{10}{l}{\# Confirmed COVID Patients in ICU:}\tabularnewline
\addlinespace[0.75ex]
~~First stage&&&13.89&15.80&13.79&15.78&15.53&15.08&14.43&13.40 \tabularnewline
~~(in millions \$)&&&(0.50)&(6.15)&(3.73)&(2.41)&(2.02)&(1.73)&(1.09)&(0.77) \tabularnewline
~~Reduced form&&&12.16&10.75&$-$0.22&4.32&4.45&4.52&0.55&$-$1.58 \tabularnewline
&&&(2.58)&(23.34)&(18.35)&(11.38)&(10.13)&(8.71)&(5.64)&(4.39) \tabularnewline
~~\$1mm of funding&1.51&0.82&0.88&0.50&$-$0.11&0.18&0.04&0.12&$-$0.13&$-$0.35 \tabularnewline
&(0.21)&(0.27)&(0.17)&(1.54)&(1.37)&(0.70)&(0.64)&(0.56)&(0.39)&(0.34) \tabularnewline
~~N&3503&3503&3503&67&181&370&514&671&1321&1868 \tabularnewline
\bottomrule %\addlinespace[1.5ex]

\end{tabularx}
\caption*{
\scriptsize{\it Note}: In this table, we estimate the effects of the funding amount on hospital-level outcomes. Column 1 presents OLS results of outcome variables on funding without controls. Column 2 controls for disproportionate patient percentage, uncompensated care per bed, and profit margin. Column 3 shows the results of 2SLS regression with no controls. In columns 4--10, we control for Approximate Propensity Score with different values of bandwidth $\delta$ on the sample with nondegenerate Approximate Propensity Scores. The first stage shows the effect of funding eligibility on the amount of relief funding received by hospitals, in millions of dollars. The reduced form shows the effect of funding eligibility on the outcome. 2SLS estimates show the effect of the amount of relief funding on outcomes. Approximate Propensity Scores are computed by averaging 10,000 simulation draws. The outcome variables are 7 day totals for the week spanning July 31st, 2020 to August 6th, 2020. Confirmed COVID patients refer to the sum of patients in inpatient beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Inpatient bed totals also include observation beds. Confirmed COVID patients in ICU refers to the sum of patients in ICU beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Robust standard errors are reported in parentheses.
}
\label{table:2sls_safetynet}
}
\end{table}


==> tables/deprecated/2SLS_safety_net_combined_OLD.tex <==
\begin{table}[!t] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Effects of Funding on Hospital Behavior}
{\tiny
\begin{tabularx}{\textwidth}{lCCCCCCCCCC}

\hline\hline\tabularnewline[-1.8ex]
{}&{OLS with}&{OLS with}&{2SLS with}&\multicolumn{7}{c}{Our Method: 2SLS with Approximate Propensity Score Controls} \tabularnewline
{}&{No}&{Covariate}&{No} \tabularnewline[-1.8ex]\cline{5-11} \tabularnewline[-1.8ex]
{}&{Controls}&{Controls}&{Controls}&{ $\delta = 0.01$}&{ $\delta = 0.025$}&{ $\delta = 0.05$}&{ $\delta = 0.075$}&{ $\delta = 0.1$}&{ $\delta = 0.25$}&{ $\delta = 0.5$} \tabularnewline
&(1)&(2)&(3)&(4)&(5)&(6)&(7)&(8)&(9)&(10)\\
\midrule\addlinespace[1.5ex]
\multicolumn{11}{l}{\# Confirmed COVID Patients}\tabularnewline
\midrule\addlinespace[1.5ex]
First stage&&&13.90&16.55&14.37&15.05&14.81&14.42&14.10&13.19 \tabularnewline
(in millions \$)&&&(0.50)&(6.11)&(3.66)&(2.33)&(1.91)&(1.64)&(1.04)&(0.75) \tabularnewline
Reduced form&&&33.97&8.82&$-$31.57&25.21&15.28&10.63&9.17&5.23 \tabularnewline
&&&(7.44)&(66.76)&(54.25)&(34.19)&(30.38)&(25.91)&(15.96)&(12.41) \tabularnewline
\$1mm of funding&4.53&2.50&2.44&0.05&$-$2.14&1.42&0.13&$-$0.03&$-$0.09&$-$0.63 \tabularnewline
&(0.63)&(0.79)&(0.50)&(4.33)&(3.97)&(2.17)&(1.97)&(1.74)&(1.12)&(0.96) \tabularnewline
N&3558&3558&3558&70&191&385&539&709&1366&1923 \tabularnewline
\midrule\addlinespace[1.5ex]
\multicolumn{10}{l}{\# Confirmed COVID Patients in ICU}\tabularnewline
\midrule\addlinespace[1.5ex]
First stage&&&13.89&15.80&13.79&15.78&15.53&15.08&14.43&13.40 \tabularnewline
(in millions \$)&&&(0.50)&(6.15)&(3.73)&(2.41)&(2.02)&(1.73)&(1.09)&(0.77) \tabularnewline
Reduced form&&&12.16&10.75&$-$0.22&4.32&4.45&4.52&0.55&$-$1.58 \tabularnewline
&&&(2.58)&(23.34)&(18.35)&(11.38)&(10.13)&(8.71)&(5.64)&(4.39) \tabularnewline
\$1mm of funding&1.51&0.82&0.88&0.50&$-$0.11&0.18&0.04&0.12&$-$0.13&$-$0.35 \tabularnewline
&(0.21)&(0.27)&(0.17)&(1.54)&(1.37)&(0.70)&(0.64)&(0.56)&(0.39)&(0.34) \tabularnewline
N&3503&3503&3503&67&181&370&514&671&1321&1868 \tabularnewline
\bottomrule %\addlinespace[1.5ex]

\end{tabularx}
\caption*{
\scriptsize{\it Notes}: In this table, we estimate the effects of the funding amount on hospital-level outcomes. Column 1 presents OLS results of outcome variables on funding without controls. Column 2 controls for disproportionate patient percentage, uncompensated care per bed, and profit margin. Column 3 shows the results of 2SLS regression with no controls. In columns 4--10, we control for Approximate Propensity Score with different values of bandwidth $\delta$ on the sample with nondegenerate Approximate Propensity Scores. The first stage shows the effect of funding eligibility on the amount of relief funding received by hospitals, in millions of dollars. The reduced form shows the effect of funding eligibility on the outcome. 2SLS estimates show the effect of the amount of relief funding on outcomes. Approximate Propensity Scores are computed by averaging 10,000 simulation draws. The outcome variables are 7 day totals for the week spanning July 31st, 2020 to August 6th, 2020. Confirmed COVID patients refer to the sum of patients in inpatient beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Inpatient bed totals also include observation beds. Confirmed COVID patients in ICU refers to the sum of patients in ICU beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Robust standard errors are reported in parentheses.
}
\label{table:2sls_safetynet}
}
\end{table}


==> tables/deprecated/2SLS_safety_net_combined_star.tex <==
\begin{table}[!t] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Effects of Funding on Hospital Behavior}
{\scriptsize
\begin{tabularx}{\textwidth}{lCCCCCCCCCC}

\hline\hline\tabularnewline[-1.8ex]
{}&{OLS with}&{OLS with}&{2SLS with}&\multicolumn{7}{c}{Our Method: 2SLS with Approximate Propensity Score Controls} \tabularnewline
{}&{No}&{Covariate}&{No} \tabularnewline[-1.8ex]\cline{5-11} \tabularnewline[-1.8ex]
{}&{Controls}&{Controls}&{Controls}&{ $\delta = 0.01$}&{ $\delta = 0.025$}&{ $\delta = 0.05$}&{ $\delta = 0.075$}&{ $\delta = 0.1$}&{ $\delta = 0.25$}&{ $\delta = 0.5$} \tabularnewline
&(1)&(2)&(3)&(4)&(5)&(6)&(7)&(8)&(9)&(10)\\
\midrule\addlinespace[1.5ex]
\multicolumn{11}{l}{\# Confirmed COVID Patients}\tabularnewline
\midrule\addlinespace[1.5ex]
First stage&&&13.90***&16.55***&14.37***&15.05***&14.81***&14.42***&14.10***&13.19*** \tabularnewline
(in millions \$)&&&(0.50)&(6.11)&(3.66)&(2.33)&(1.91)&(1.64)&(1.04)&(0.75) \tabularnewline
Reduced Form&&&33.97***&8.82&$-$31.57&25.21&15.28&10.63&9.17&5.23 \tabularnewline
&&&(7.44)&(66.76)&(54.25)&(34.19)&(30.38)&(25.91)&(15.96)&(12.41) \tabularnewline
\$1mm of funding&4.53***&2.50***&2.44***&0.05&$-$2.14&1.42&0.13&$-$0.03&$-$0.09&$-$0.63 \tabularnewline
&(0.63)&(0.79)&(0.50)&(4.33)&(3.97)&(2.17)&(1.97)&(1.74)&(1.12)&(0.96) \tabularnewline
N&3558&3558&3558&70&191&385&539&709&1366&1923 \tabularnewline
\midrule\addlinespace[1.5ex]
\multicolumn{10}{l}{\# Confirmed COVID Patients in ICU}\tabularnewline
\midrule\addlinespace[1.5ex]
First stage&&&13.89***&15.80**&13.79***&15.78***&15.53***&15.08***&14.43***&13.40*** \tabularnewline
(in millions \$)&&&(0.50)&(6.15)&(3.73)&(2.41)&(2.02)&(1.73)&(1.09)&(0.77) \tabularnewline
Reduced Form&&&12.16***&10.75&$-$0.22&4.32&4.45&4.52&0.55&$-$1.58 \tabularnewline
&&&(2.58)&(23.34)&(18.35)&(11.38)&(10.13)&(8.71)&(5.64)&(4.39) \tabularnewline
\$1mm of funding&1.51***&0.82***&0.88***&0.50&$-$0.11&0.18&0.04&0.12&$-$0.13&$-$0.35 \tabularnewline
&(0.21)&(0.27)&(0.17)&(1.54)&(1.37)&(0.70)&(0.64)&(0.56)&(0.39)&(0.34) \tabularnewline
N&3503&3503&3503&67&181&370&514&671&1321&1868 \tabularnewline
\bottomrule %\addlinespace[1.5ex]

\end{tabularx}
\caption*{
\scriptsize{\it Notes}: In this table, we estimate the effects of the funding amount on hospital-level outcomes. Column 1 presents OLS results of outcome variables on funding without controls. Column 2 controls for disproportionate patient percentage, uncompensated care per bed, and profit margin. Column 3 shows the results of 2SLS regression with no controls. In columns 4--10, we control for Approximate Propensity Score with different values of bandwidth $\delta$ on the sample with nondegenerate Approximate Propensity Scores. The first stage shows the effect of funding eligibility on the amount of relief funding received by hospitals, in millions of dollars. The reduced form shows the effect of funding eligibility on the outcome. 2SLS estimates show the effect of relief funding on outcomes. Approximate Propensity Scores are computed by averaging 10,000 simulation draws. The outcome variables are 7 day totals for the week spanning July 31st, 2020 to August 6th, 2020. Confirmed COVID patients refer to the sum of patients in inpatient beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Inpatient bed totals also include observation beds. Confirmed COVID patients in ICU refers to the sum of patients in ICU beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Robust standard errors are reported in parentheses. */**/*** indicate $p <$ 0.10/0.05/0.01.
}
\label{table:2sls_safetynet}
}
\end{table}


==> tables/deprecated/2SLS_safety_net_indicator_10.tex <==
\begin{table}[h] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Effects of Funding on Hospital Behavior}
{\scriptsize
\begin{tabularx}{\linewidth}{lCCCCCCCCCC}

\begin{comment}
\hline\hline\tabularnewline[-1.8ex]
{}&{OLS with}&{OLS with}&{2SLS with}&\multicolumn{7}{c}{Our Method: 2SLS with Approximate Propensity Score Controls} \tabularnewline
{}&{No}&{Covariate}&{No} \tabularnewline[-1.8ex]\cline{5-11} \tabularnewline[-1.8ex]
{}&{Controls}&{Controls}&{Controls}&{ $\delta = 0.01$}&{ $\delta = 0.025$}&{ $\delta = 0.05$}&{ $\delta = 0.075$}&{ $\delta = 0.1$}&{ $\delta = 0.25$}&{ $\delta = 0.5$} \tabularnewline
&(1)&(2)&(3)&(4)&(5)&(6)&(7)&(8)&(9)&(10)\\
\midrule\addlinespace[1.5ex]
\multicolumn{11}{l}{\# Confirmed/Suspected COVID Patients}\tabularnewline 
\midrule\addlinespace[1.5ex]
First stage&&&0.42***&0.30*&0.34***&0.39***&0.38***&0.37***&0.41***&0.39*** \tabularnewline
&&&(0.02)&(0.18)&(0.12)&(0.08)&(0.07)&(0.06)&(0.04)&(0.03) \tabularnewline
> \$10mm funding&150.8***&90.0***&91.22***&$-$50.94&$-$73.30&$-$112.64&$-$150.62&$-$110.33&5.02&$-$10.45 \tabularnewline
&(15.43)&(19.82)&(19.07)&(283.57)&(214.76)&(182.25)&(169.64)&(136.88)&(54.31)&(40.31) \tabularnewline
N&3532&3532&3532&73&195&392&547&719&1389&1947 \tabularnewline
\midrule\addlinespace[1.5ex] 
\multicolumn{11}{l}{\# Confirmed COVID Patients}\tabularnewline 
\midrule\addlinespace[1.5ex] \tabularnewline
First stage&&&0.42***&0.35*&0.40***&0.43***&0.41***&0.39***&0.41***&0.40*** \tabularnewline
&&&(0.02)&(0.19)&(0.12)&(0.08)&(0.07)&(0.06)&(0.04)&(0.03) \tabularnewline
> \$10mm funding&127.4***&76.0***&80.67***&2.41&$-$76.82&49.63&4.75&$-$0.99&$-$3.13&$-$20.83 \tabularnewline
&(14.08)&(17.32)&(16.53)&(202.58)&(143.63)&(75.69)&(70.83)&(63.99)&(38.55)&(32.19) \tabularnewline
N&3558&3558&3558&70&191&385&539&709&1366&1923 \tabularnewline
\midrule\addlinespace[1.5ex] 
\multicolumn{11}{l}{\# Confirmed/Suspected COVID Patients in ICU}\tabularnewline 
\midrule\addlinespace[1.5ex] 
First stage&&&0.42***&0.29*&0.36***&0.46***&0.44***&0.41***&0.43***&0.40*** \tabularnewline
&&&(0.02)&(0.17)&(0.11)&(0.08)&(0.07)&(0.06)&(0.04)&(0.03) \tabularnewline
> \$10mm funding&47.0***&27.5***&31.14***&47.19&26.74&12.34&$-$1.89&5.63&$-$1.06&$-$10.48 \tabularnewline
&(4.95)&(6.38)&(6.04)&(72.38)&(47.41)&(25.11)&(24.41)&(21.47)&(13.42)&(11.83) \tabularnewline
N&3445&3445&3445&72&186&374&520&678&1314&1846 \tabularnewline
\midrule\addlinespace[1.5ex] 
\multicolumn{11}{l}{\# Confirmed COVID Patients in ICU}\tabularnewline 
\midrule\addlinespace[1.5ex]
First stage&&&0.43***&0.33*&0.38***&0.46***&0.45***&0.43***&0.44***&0.41*** \tabularnewline
&&&(0.02)&(0.19)&(0.12)&(0.09)&(0.07)&(0.06)&(0.04)&(0.03) \tabularnewline
> \$10mm funding&41.6***&23.9***&28.37***&24.31&$-$4.01&6.01&1.44&4.36&$-$4.44&$-$11.29 \tabularnewline
&(4.79)&(5.94)&(5.65)&(72.70)&(49.11)&(23.85)&(22.12)&(19.64)&(12.89)&(10.99) \tabularnewline
N&3503&3503&3503&67&181&370&514&671&1321&1868 \tabularnewline
\bottomrule

\end{tabularx}
\caption*{
\scriptsize{\it Notes}: In this table we regress outcomes at the hospital level on a indicator for receiving more than \$10mm in safety net funding. Column 1 presents the results of OLS regression without controls. Column 2 presents the results of OLS controlling for disproportionate patient percentage, uncompensated care per bed, and profit margin.  In columns 3$-$10, we instrument the funding treatment with eligibility to receive this funding and present the results of 2SLS regressions. In columns 3$-$10, the first stage shows the effect of funding eligibility on the funding treatment. Column 3 shows the results of a 2SLS regression with no controls.  In columns 4$-$10, we control for the Approximate Propensity Score with different values of bandwidth $\delta$ on the sample with nondegenerate Approximate Propensity Scores. All Approximate Propensity Scores are computed by averaging 10,000 simulation draws. The outcome variables are the 7 day totals for the week spanning July 31st, 2020 to August 6th, 2020. Confirmed or Suspected COVID patients refer to the sum of patients in inpatient beds with lab-confirmed/suspected COVID-19. Confirmed COVID patients refer to the sum of patients in inpatient beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Inpatient bed totals also include observation beds. Similarly, Confirmed/Suspected COVID patients in ICU refer to the sum of patients in ICU beds with lab-confirmed or suspected COVID-19. Confirmed COVID patients in ICU refers to the sum of patients in ICU beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Robust standard errors are reported in parentheses. */**/*** indicate p < 0.10/0.05/0.01
}
\label{table:2sls_safetynet_indicator10}
}
\end{comment}
\end{table}


==> tables/deprecated/Covariate_balance_safety_net.tex <==
%\newgeometry{left=0.4in, right=0.4in, top=1in}
\begin{table}[!t] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Covariate Balance Regressions}
{\scriptsize
\begin{tabularx}{\textwidth}{lCCCCCCCCC}

\toprule
{}&{}&{}&\multicolumn{7}{c}{Our Method: OLS with Approximate Propensity Score Controls} \tabularnewline[-2ex] {}&{Mean (Ineli-}&{OLS with}&\tabularnewline[-1ex] \cline{4-10} \tabularnewline[-2ex]
{}&{gible Hospitals)}&{No Controls}&{ $\delta = 0.01$}&{ $\delta = 0.025$}&{ $\delta = 0.05$}&{ $\delta = 0.075$}&{ $\delta = 0.1$}&{ $\delta = 0.25$}&{ $\delta = 0.5$} \tabularnewline
&{(1)}&{(2)}&{(3)}&{(4)}&{(5)}&{(6)}&{(7)}&{(8)}&{(9)} \\%\tabularnewline
\midrule\addlinespace[1.5ex]
%\tabularnewline[-1.8ex]
\multicolumn{10}{c}{Panel A: Determinants of Funding Eligibility} \\ \tabularnewline[-2ex]
Profit margin&.04&$-$0.11&$-$0.03&$-$0.00&0.02&0.01&0.02&0.05&0.06 \tabularnewline
&&(0.01)&(0.06)&(0.04)&(0.03)&(0.03)&(0.02)&(0.01)&(0.01) \tabularnewline
&&N=4633&N=89&N=239&N=485&N=671&N=879&N=1726&N=2368 \tabularnewline
Uncompensated&56,556&19,540&4,905&10,761&$-$4,229&$-$9,600&$-$11,001&$-$8,005&$-$6,121 \tabularnewline
%&56556.02&19,540.28&4,905.22&10,760.57&$-$4,229.12&$-$9,599.98&$-$11,001.30&$-$8,005.95&$-$6,121.90 \tabularnewline
care per bed (\$)&&(3,827)&(12,161)&(10,356)&(8,611)&(7,651)&(6,976)&(4,498)&(3,660) \tabularnewline
%&&(3,827.22)&(12,161.31)&(10,355.61)&(8,611.29)&(7,651.29)&(6,976.02)&(4,498.41)&(3,660.04) \tabularnewline
&&N=4633&N=89&N=239&N=485&N=671&N=879&N=1726&N=2368 \tabularnewline
Disproportionate&.18&0.21&$-$0.09&$-$0.09&$-$0.09&$-$0.08&$-$0.08&$-$0.06&$-$0.07 \tabularnewline
patient percentage&&(0.01)&(0.09)&(0.07)&(0.07)&(0.06)&(0.05)&(0.02)&(0.02) \tabularnewline
&&N=4633&N=89&N=239&N=485&N=671&N=879&N=1726&N=2368 \tabularnewline\tabularnewline
%\tabularnewline[-0.5ex]
\multicolumn{10}{c}{Panel B: Other Hospital Characteristics} \\ \tabularnewline[-2ex]
Full time employees&897.32&454.26&2,670.64&387.75&37.55&90.96&64.41&214.79&115.94 \tabularnewline
&&(69.23)&(1,652.55)&(997.64)&(668.32)&(515.72)&(414.25)&(218.77)&(143.35) \tabularnewline
&&N=4626&N=89&N=238&N=484&N=670&N=878&N=1723&N=2365 \tabularnewline
Medicare net revenue&20.04&18.36&35.34&$-$7.92&$-$6.16&$-$1.47&2.41&4.70&$-$0.47 \tabularnewline
(in millions \$)&&(2.39)&(29.74)&(18.36)&(14.34)&(12.09)&(10.81)&(6.63)&(4.68) \tabularnewline
&&N=4511&N=88&N=238&N=483&N=667&N=875&N=1684&N=2323 \tabularnewline
Occupancy&.44&0.07&0.19&0.07&$-$0.00&0.01&0.01&0.03&0.04 \tabularnewline
&&(0.01)&(0.09)&(0.06)&(0.04)&(0.04)&(0.03)&(0.02)&(0.01) \tabularnewline
&&N=4624&N=89&N=239&N=485&N=671&N=879&N=1726&N=2368 \tabularnewline
Operating margin&.02&$-$0.11&$-$0.03&0.00&0.02&0.02&0.03&0.06&0.07 \tabularnewline
&&(0.01)&(0.06)&(0.04)&(0.03)&(0.03)&(0.03)&(0.02)&(0.01) \tabularnewline
&&N=4541&N=88&N=238&N=477&N=661&N=868&N=1676&N=2314 \tabularnewline
Beds&134.6&53.75&198.67&35.86&2.93&7.02&11.93&17.47&8.92 \tabularnewline
&&(7.05)&(105.74)&(66.42)&(47.75)&(39.24)&(33.06)&(20.05)&(14.46) \tabularnewline
&&N=4633&N=89&N=239&N=485&N=671&N=879&N=1726&N=2368 \tabularnewline
Costs per discharge&66.28&$-$49.95&3.83&3.37&1.65&$-$6.42&$-$0.88&6.06&6.76 \tabularnewline
(in thousands \$)&&(17.93)&(2.18)&(1.49)&(1.23)&(8.12)&(2.58)&(4.63)&(5.09) \tabularnewline
&&N=3539&N=89&N=239&N=485&N=671&N=879&N=1726&N=2368 \tabularnewline
p-value joint significance&&0&.74&.457&.87&.745&.286&0&0 \tabularnewline
\bottomrule %\addlinespace[1.5ex]

\end{tabularx}
\caption*{
\scriptsize{\it Note}: This table shows the results of the covariate balance regressions at the hospital level. The dependent variables for these regressions are drawn from the
Healthcare Cost Report Information System for the financial year 2018. Disproportionate patient percentage, profit margin and uncompensated care per bed
are used to determine the hospital’s funding eligibility. Other dependent variables shown indicate the financial health and utilization of the hospitals.
In column 2, we regress the dependent variables on the eligibility of the hospital with no controls. In columns 3–9, we regress the dependent variables on funding eligibility controlling for the Approximate Propensity Score with different values of bandwidth $\delta$. All Approximate Propensity Scores are
computed by averaging 10,000 simulation draws. Column 1 shows the mean of dependent variables for hospitals that are ineligible to receive safety net funding.
Robust standard errors are reported in the parenthesis and the number of observations is reported separately for each regression. The last row reports the $p$-value
of the joint significance test.
}
}
\label{table:CBR}
\end{table}
%\restoregeometry


==> tables/deprecated/Covariate_balance_safety_net_star.tex <==
%\newgeometry{left=0.4in, right=0.4in, top=1in}
\begin{table}[!t] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Covariate Balance Regressions}
{\scriptsize
\begin{tabularx}{\textwidth}{lCCCCCCCCC}

\toprule
{}&{}&{}&\multicolumn{7}{c}{Our Method: OLS with Approximate Propensity Score Controls} \tabularnewline[-2ex] {}&{Mean (Ineli-}&{OLS with}&\tabularnewline[-1ex] \cline{4-10} \tabularnewline[-2ex]
{}&{gible Hospitals)}&{No Controls}&{ $\delta = 0.01$}&{ $\delta = 0.025$}&{ $\delta = 0.05$}&{ $\delta = 0.075$}&{ $\delta = 0.1$}&{ $\delta = 0.25$}&{ $\delta = 0.5$} \tabularnewline
&{(1)}&{(2)}&{(3)}&{(4)}&{(5)}&{(6)}&{(7)}&{(8)}&{(9)} \tabularnewline
\midrule\addlinespace[1.5ex]
\tabularnewline[-0.5ex]
\multicolumn{10}{c}{Panel A: Determinants of Funding Eligibility} \\ \tabularnewline[-0.5ex]
Profit margin&.04&$-$0.11***&$-$0.03&$-$0.00&0.02&0.01&0.02&0.05***&0.06*** \tabularnewline
&&(0.01)&(0.06)&(0.04)&(0.03)&(0.03)&(0.02)&(0.01)&(0.01) \tabularnewline
&&N=4633&N=89&N=239&N=485&N=671&N=879&N=1726&N=2368 \tabularnewline
Uncompensated&56556&19,540***&4,905&10,761&$-$4,229&$-$9,600&$-$11,001&$-$8,005*&$-$6,121* \tabularnewline
%&56556.02&19,540.28***&4,905.22&10,760.57&$-$4,229.12&$-$9,599.98&$-$11,001.30&$-$8,005.95*&$-$6,121.90* \tabularnewline
care per bed (\$)&&(3,827)&(12,161)&(10,356)&(8,611)&(7,651)&(6,976)&(4,498)&(3,660) \tabularnewline
%&&(3,827.22)&(12,161.31)&(10,355.61)&(8,611.29)&(7,651.29)&(6,976.02)&(4,498.41)&(3,660.04) \tabularnewline
&&N=4633&N=89&N=239&N=485&N=671&N=879&N=1726&N=2368 \tabularnewline
Disproportionate&.18&0.21***&$-$0.09&$-$0.09&$-$0.09&$-$0.08&$-$0.08*&$-$0.06**&$-$0.07*** \tabularnewline
patient percentage&&(0.01)&(0.09)&(0.07)&(0.07)&(0.06)&(0.05)&(0.02)&(0.02) \tabularnewline
&&N=4633&N=89&N=239&N=485&N=671&N=879&N=1726&N=2368 \tabularnewline
\tabularnewline[-0.5ex]
\multicolumn{10}{c}{Panel B: Other Hospital Characteristics} \\ \tabularnewline[-0.5ex]
Full time employees&897.32&454.26***&2,670.64&387.75&37.55&90.96&64.41&214.79&115.94 \tabularnewline
&&(69.23)&(1,652.55)&(997.64)&(668.32)&(515.72)&(414.25)&(218.77)&(143.35) \tabularnewline
&&N=4626&N=89&N=238&N=484&N=670&N=878&N=1723&N=2365 \tabularnewline
Medicare net revenue&20.04&18.36***&35.34&$-$7.92&$-$6.16&$-$1.47&2.41&4.70&$-$0.47 \tabularnewline
(in millions \$)&&(2.39)&(29.74)&(18.36)&(14.34)&(12.09)&(10.81)&(6.63)&(4.68) \tabularnewline
&&N=4511&N=88&N=238&N=483&N=667&N=875&N=1684&N=2323 \tabularnewline
Occupancy&.44&0.07***&0.19**&0.07&$-$0.00&0.01&0.01&0.03*&0.04*** \tabularnewline
&&(0.01)&(0.09)&(0.06)&(0.04)&(0.04)&(0.03)&(0.02)&(0.01) \tabularnewline
&&N=4624&N=89&N=239&N=485&N=671&N=879&N=1726&N=2368 \tabularnewline
Operating margin&.02&$-$0.11***&$-$0.03&0.00&0.02&0.02&0.03&0.06***&0.07*** \tabularnewline
&&(0.01)&(0.06)&(0.04)&(0.03)&(0.03)&(0.03)&(0.02)&(0.01) \tabularnewline
&&N=4541&N=88&N=238&N=477&N=661&N=868&N=1676&N=2314 \tabularnewline
Beds&134.6&53.75***&198.67*&35.86&2.93&7.02&11.93&17.47&8.92 \tabularnewline
&&(7.05)&(105.74)&(66.42)&(47.75)&(39.24)&(33.06)&(20.05)&(14.46) \tabularnewline
&&N=4633&N=89&N=239&N=485&N=671&N=879&N=1726&N=2368 \tabularnewline
Costs per discharge&66.28&$-$49.95***&3.83*&3.37**&1.65&$-$6.42&$-$0.88&6.06&6.76 \tabularnewline
(in thousands \$)&&(17.93)&(2.18)&(1.49)&(1.23)&(8.12)&(2.58)&(4.63)&(5.09) \tabularnewline
&&N=3539&N=89&N=239&N=485&N=671&N=879&N=1726&N=2368 \tabularnewline
p-value joint significance&&0&.74&.457&.87&.745&.286&0&0 \tabularnewline
\bottomrule %\addlinespace[1.5ex]

\end{tabularx}
\caption*{
\scriptsize{\it Notes}: This table shows the results of the covariate balance regressions at the hospital level. The dependent variables for these regressions are drawn from the
Healthcare Cost Report Information System for the financial year 2018. Disproportionate patient percentage, profit margin and uncompensated care per bed
are used to determine the hospital’s funding eligibility. Other dependent variables shown indicate the financial health and utilization of the hospitals.
In column 2, we regress the dependent variables on the eligibility of the hospital with no controls. In columns 3–9, we regress the dependent variables on funding eligibility controlling for the Approximate Propensity Score with different values of bandwidth $\delta$. All Approximate Propensity Scores are
computed by averaging 10,000 simulation draws. Column 1 shows the mean of dependent variables for hospitals that are ineligible to receive safety net funding.
Robust standard errors are reported in the parenthesis and the number of observations is reported separately for each regression. The last row reports the $p$-value
of the joint significance test. */**/*** indicate $p <$ 0.10/0.05/0.01.
}
}
\label{table:CBR}
\end{table}
%\restoregeometry


==> tables/deprecated/Descriptive_stats.tex <==
\begin{table}[!t] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}
\caption{Hospital Characteristics and Outcomes}
{\scriptsize
\begin{tabularx}{\textwidth}{lCCCC}

\hline\tabularnewline[-1.8ex]
{}&{All}&{Ineligible}&{Eligible}&{Hospitals w/} \\
{}&{}&{Hospitals}&{Hospitals}&{APS $\in$ (0,1)} \\
\midrule\addlinespace[1.5ex]
\multicolumn{5}{c}{Panel A: Outcome Variable Means} \\ \tabularnewline[-2.0ex]
\# Confirmed/Suspected COVID Patients&105.59&98.41&136.61&125.19 \tabularnewline
\# Confirmed COVID Patients&80.10&73.86&107.83&86.78 \tabularnewline
\# Confirmed/Suspected COVID Patients in ICU&31.37&28.92&42.10&36.84 \tabularnewline
\# Confirmed COVID Patients in ICU&26.62&24.41&36.56&31.41 \tabularnewline
N&4,008&3,293&715&429 \tabularnewline\tabularnewline
\multicolumn{5}{c}{Panel B: Hospital Characteristics Means} \tabularnewline\tabularnewline[-2.0ex]
Beds&143.66&134.60&188.35&206.47 \tabularnewline
Interns and residents (full-time equivalents) per bed&.06&.05&.11&.09 \tabularnewline
Adult and pediatric hospital beds&120.26&113.29&154.66&170.49 \tabularnewline
Ownership: Proprietary (for-profit)&.19&.20&.18&.15 \tabularnewline
Ownership: Governmental&.22&.22&.23&.16 \tabularnewline
Ownership: Voluntary (non-profit)&.58&.58&.59&.68 \tabularnewline
Inpatient length of stay&9.21&10.14&4.66&4.38 \tabularnewline
Employees on payroll (full-time equivalents)&973.90&897.31&1351.57&1525.06 \tabularnewline
Disproportionate patient percentage&.21&.18&.38&.36 \tabularnewline
Uncompensated care per bed (\$) &59,850.00&56,556.03&76,096.31&45,996.48 \tabularnewline
Profit margin&.02&.04&$-$.07&$-$.03 \tabularnewline
N&4,633&3,852&781&485 \tabularnewline
\bottomrule %\addlinespace[1.5ex]
\end{tabularx}
\caption*{
\scriptsize {\it Note}: This table reports averages of outcome variables and hospital characteristics by funding eligibility. %A safety net hospital is defined as any acute care hospital with disproportionate patient percentage of 20.2\% or greater, annual uncompensated care of at least \$25,000 per bed and profit margin of 3.0\% or less. 
Panel A reports the outcome variable means. Outcome variable estimates are 7 day sums for the week spanning July 31st 2020 to August 6th 2020.  Confirmed or Suspected COVID patients refer to the sum of patients in inpatient beds with lab-confirmed/suspected COVID. Confirmed COVID patients refer to the sum of patients in inpatient beds with lab-confirmed COVID, including those with both lab-confirmed COVID and influenza. Inpatient bed totals also include observation beds. Similarly, Confirmed/Suspected COVID patients in ICU refer to the sum of patients in ICU beds with lab-confirmed or suspected COVID. Confirmed COVID patients in ICU refers to the sum of patients in ICU beds with lab-confirmed COVID, including those with both lab-confirmed COVID and influenza. Panel B reports the means for hospital characteristics for the financial year 2018. Column 1 shows the means for all hospitals. Columns 2 and 3 show the means for hospitals that are ineligible and eligible to receive funding, respectively. Column 4 shows the means for the hospitals with nondegenerate Approximate Propensity Score with bandwidth $\delta=0.05$. Approximate Propensity Score is computed by averaging 10,000 simulation draws. 
}
}
\label{tbl:descriptives}
\end{table}


==> tables/deprecated/Descriptive_stats_OLD.tex <==
\begin{table}[!t] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}
\caption{Hospital Characteristics and Outcomes}
{\scriptsize
\begin{tabularx}{\textwidth}{lCCCC}

\hline\hline\tabularnewline[-1.8ex]
{}&{All}&{Ineligible}&{Eligible}&{Hospitals w/} \\
{}&{}&{Hospitals}&{Hospitals}&{APS $\in$ (0,1)} \\
\midrule\addlinespace[1.5ex]
\multicolumn{5}{c}{Panel A: Outcome Variable Means} \\ \tabularnewline[-2.0ex]
\# Confirmed/Suspected COVID Patients&105.59&98.41&136.61&125.19 \tabularnewline
\# Confirmed COVID Patients&80.10&73.86&107.83&86.78 \tabularnewline
\# Confirmed/Suspected COVID Patients in ICU&31.37&28.92&42.10&36.84 \tabularnewline
\# Confirmed COVID Patients in ICU&26.62&24.41&36.56&31.41 \tabularnewline
N&4,008&3,293&715&429 \tabularnewline\tabularnewline
\multicolumn{5}{c}{Panel B: Hospital Characteristics Means} \tabularnewline\tabularnewline[-2.0ex]
Beds&143.66&134.60&188.35&206.47 \tabularnewline
Interns and residents (full-time equivalents) per bed&.06&.05&.11&.09 \tabularnewline
Adult and pediatric hospital beds&120.26&113.29&154.66&170.49 \tabularnewline
Ownership: Proprietary (for-profit)&.19&.20&.18&.15 \tabularnewline
Ownership: Governmental&.22&.22&.23&.16 \tabularnewline
Ownership: Voluntary (non-profit)&.58&.58&.59&.68 \tabularnewline
Inpatient length of stay&9.21&10.14&4.66&4.38 \tabularnewline
Employees on payroll (full-time equivalents)&973.90&897.31&1351.57&1525.06 \tabularnewline
Disproportionate patient percentage&.21&.18&.38&.36 \tabularnewline
Uncompensated care per bed (\$) &59,850.00&56,556.03&76,096.31&45,996.48 \tabularnewline
Profit margin&.02&.04&$-$.07&$-$.03 \tabularnewline
N&4,633&3,852&781&485 \tabularnewline
\bottomrule %\addlinespace[1.5ex]
\end{tabularx}
\caption*{
\scriptsize {\it Notes}: This table reports averages of outcome variables and hospital characteristics by funding eligibility. %A safety net hospital is defined as any acute care hospital with disproportionate patient percentage of 20.2\% or greater, annual uncompensated care of at least \$25,000 per bed and profit margin of 3.0\% or less. 
Panel A reports the outcome variable means. Outcome variable estimates are 7 day sums for the week spanning July 31st 2020 to August 6th 2020.  Confirmed or Suspected COVID patients refer to the sum of patients in inpatient beds with lab-confirmed/suspected COVID. Confirmed COVID patients refer to the sum of patients in inpatient beds with lab-confirmed COVID, including those with both lab-confirmed COVID and influenza. Inpatient bed totals also include observation beds. Similarly, Confirmed/Suspected COVID patients in ICU refer to the sum of patients in ICU beds with lab-confirmed or suspected COVID. Confirmed COVID patients in ICU refers to the sum of patients in ICU beds with lab-confirmed COVID, including those with both lab-confirmed COVID and influenza. Panel B reports the means for hospital characteristics for the financial year 2018. Column 1 shows the means for all hospitals. Columns 2 and 3 show the means for hospitals that are ineligible and eligible to receive funding, respectively. Column 4 shows the means for the hospitals with nondegenerate Approximate Propensity Score with bandwidth $\delta=0.05$. Approximate Propensity Score is computed by averaging 10,000 simulation draws. 
}
}
\label{tbl:descriptives}
\end{table}


==> tables/deprecated/differential_attrition.tex <==

\begin{table}[!ht] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Differential Attrition}
{\scriptsize
\begin{tabularx}{\textwidth}{lCCCCCCCCCC}

\toprule
{}&{}&{}&\multicolumn{7}{c}{Our Method with Approximate Propensity Score Controls}\\
{}&{Ineligible}&{No}&\\\cline{4-10}
{}&{Hospitals}&{Controls}&
{ $\delta = 0.01$}&{ $\delta = 0.025$}&{ $\delta = 0.05$}&{ $\delta = 0.075$}&{ $\delta = 0.1$}&{ $\delta = 0.25$}&{ $\delta = 0.5$} \tabularnewline
{}&{(1)}&{(2)}&{(3)}&{(4)}&{(5)}&{(6)}&{(7)}&{(8)}&{(9)}\tabularnewline
\midrule\addlinespace[1.5ex]
\#Confirmed/Suspected&.745&0.11&0.23&$-$0.03&0.03&0.04&0.05&0.04&0.09 \tabularnewline
Covid Patients&&(0.01)&(0.17)&(0.11)&(0.08)&(0.06)&(0.06)&(0.04)&(0.03) \tabularnewline
&&N=4633&N=89&N=239&N=485&N=671&N=879&N=1726&N=2368 \tabularnewline
\#Confirmed Covid Patients&.754&0.08&0.12&$-$0.07&$-$0.04&$-$0.01&0.01&0.04&0.10 \tabularnewline
&&(0.01)&(0.21)&(0.12)&(0.08)&(0.07)&(0.06)&(0.04)&(0.03) \tabularnewline
&&N=4633&N=89&N=239&N=485&N=671&N=879&N=1726&N=2368 \tabularnewline
\#Confirmed/Suspected&.728&0.09&0.20&$-$0.01&$-$0.13&$-$0.11&$-$0.07&0.01&0.08 \tabularnewline
Covid Patients in ICU&&(0.02)&(0.16)&(0.11)&(0.08)&(0.07)&(0.06)&(0.04)&(0.03) \tabularnewline
&&N=4633&N=89&N=239&N=485&N=671&N=879&N=1726&N=2368 \tabularnewline
\#Confirmed Covid Patients&.744&0.07&0.27&0.16&0.03&$-$0.05&$-$0.03&0.01&0.06 \tabularnewline
in ICU&&(0.02)&(0.20)&(0.13)&(0.09)&(0.07)&(0.06)&(0.04)&(0.03) \tabularnewline
&&N=4633&N=89&N=239&N=485&N=671&N=879&N=1726&N=2368 \tabularnewline
\bottomrule %\addlinespace[1.5ex]

\end{tabularx}
\caption*{
\scriptsize {\it {Note}}: This table reports differential safety net eligibility effects on the availability of outcome data at the hospital level. Column 1 presents the average of the  availability indicators of the outcome variables for the ineligible hospitals. In column 2, we regress the availability indicator on dummy for safety net eligibility without any controls. In columns 3-9, we run this regression controlling for the Approximate Propensity Score with different values of bandwidth $\delta$ on the sample with nondegenerate Approximate Propensity Score. All Approximate Propensity Scores are computed by averaging 10,000 simulation draws. 
The outcome variables are the 7 day totals for the week spanning July 31st, 2020 to August 6th, 2020. Confirmed or Suspected COVID patients refer to the sum of patients in inpatient beds with lab-confirmed/suspected COVID-19. Confirmed COVID patients refer to the sum of patients in inpatient beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Inpatient bed totals also include observation beds. Similarly, Confirmed/Suspected COVID patients in ICU refer to the sum of patients in ICU beds with lab-confirmed or suspected COVID-19. Confirmed COVID patients in ICU refers to the sum of patients in ICU beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Robust standard errors are reported in parenthesis.
}
\label{table:differential_attrition}
}

\end{table}



==> tables/deprecated/differential_attrition_star.tex <==

\begin{table}[!ht] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Differential Attrition}
{\scriptsize
\begin{tabularx}{\textwidth}{lCCCCCCCCCC}

\toprule
{}&{}&{}&\multicolumn{7}{c}{Our Method with Approximate Propensity Score Controls}\\
{}&{Ineligible}&{No}&\\\cline{4-10}
{}&{Hospitals}&{Controls}&
{ $\delta = 0.01$}&{ $\delta = 0.025$}&{ $\delta = 0.05$}&{ $\delta = 0.075$}&{ $\delta = 0.1$}&{ $\delta = 0.25$}&{ $\delta = 0.5$} \tabularnewline
{}&{(1)}&{(2)}&{(3)}&{(4)}&{(5)}&{(6)}&{(7)}&{(8)}&{(9)}\tabularnewline
\midrule\addlinespace[1.5ex]
\#Confirmed/Suspected&.745&38.19***&$-$15.51&$-$24.80&$-$44.34&$-$57.95&$-$40.34&2.05&$-$4.08 \tabularnewline
Covid Patients&&(8.55)&(85.67)&(70.81)&(70.09)&(63.06)&(48.58)&(22.20)&(15.67) \tabularnewline
&&N=3532&N=73&N=195&N=392&N=547&N=719&N=1389&N=1947 \tabularnewline
\#Confirmed Covid Patients&.754&33.97***&0.85&$-$30.81&21.32&1.96&$-$0.39&$-$1.28&$-$8.25 \tabularnewline
&&(7.44)&(73.28)&(55.22)&(33.46)&(29.41)&(25.14)&(15.75)&(12.56) \tabularnewline
&&N=3558&N=70&N=191&N=385&N=539&N=709&N=1366&N=1923 \tabularnewline
\#Confirmed/Suspected&.728&13.18***&13.68&9.54&5.71&$-$0.83&2.34&$-$0.46&$-$4.21 \tabularnewline
Covid Patients in ICU&&(2.74)&(23.41)&(17.74)&(11.91)&(10.68)&(9.01)&(5.78)&(4.64) \tabularnewline
&&N=3445&N=72&N=186&N=374&N=520&N=678&N=1314&N=1846 \tabularnewline
\#Confirmed Covid Patients&.744&12.16***&7.97&$-$1.54&2.79&0.65&1.87&$-$1.94&$-$4.66 \tabularnewline
in ICU&&(2.58)&(25.63)&(18.89)&(11.25)&(9.97)&(8.52)&(5.57)&(4.43) \tabularnewline
&&N=3503&N=67&N=181&N=370&N=514&N=671&N=1321&N=1868 \tabularnewline
\bottomrule %\addlinespace[1.5ex]

\end{tabularx}
\caption*{
\scriptsize {\it {Notes}}: This table reports differential safety net eligibility effects on the availability of outcome data at the hospital level. Column 1 presents the average of the  availability indicators of the outcome variables for the ineligible hospitals. In column 2, we regress the availability indicator on dummy for safety net eligibility without any controls. In columns 3-9, we run this regression controlling for the Approximate Propensity Score with different values of bandwidth $\delta$ on the sample with nondegenerate Approximate Propensity Score. All Approximate Propensity Scores are computed by averaging 10,000 simulation draws. 
The outcome variables are the 7 day totals for the week spanning July 31st, 2020 to August 6th, 2020. Confirmed or Suspected COVID patients refer to the sum of patients in inpatient beds with lab-confirmed/suspected COVID-19. Confirmed COVID patients refer to the sum of patients in inpatient beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Inpatient bed totals also include observation beds. Similarly, Confirmed/Suspected COVID patients in ICU refer to the sum of patients in ICU beds with lab-confirmed or suspected COVID-19. Confirmed COVID patients in ICU refers to the sum of patients in ICU beds with lab-confirmed COVID-19, including those with both lab-confirmed COVID-19 and influenza. Robust standard errors are reported in parenthesis.
*/**/*** indicate $p <$ 0.10/0.05/0.01.
}
\label{table:differential_attrition}
}

\end{table}



==> tables/deprecated/simulation_OLD.tex <==
%\newgeometry{margin=0.8in}
\begin{table}[bp] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Bias, RMSE, and SD of Estimators and Coverage of 95\% Confidence Intervals}
{\scriptsize
\begin{tabularx}{\textwidth}{lCCCCCCCC}

\toprule
{}&{}&{}&\multicolumn{6}{c}{Our Method: 2SLS with Approximate Propensity Score Controls} \tabularnewline {}&{OLS}&{2SLS}&\tabularnewline[-2.5ex] \cline{4-9} \tabularnewline
{}&{with No Controls}&{with $A(X_i)$ Controls}&{$\delta = 0.01$}&{$\delta = 0.05$}&{$\delta = 0.1$}&{$\delta = 0.25$}&{$\delta = 0.5$}&{$\delta = 1$} \tabularnewline
\midrule\addlinespace[1.5ex]
\multicolumn{9}{c}{Panel A: Homogeneous Conditional Effects (Model A)} \tabularnewline
\addlinespace[1.5ex]
\multicolumn{9}{l}{Estimand: ATE = 0} \tabularnewline
\addlinespace[0.75ex]
~~Bias&0.663&0.558&0.564&0.615&0.652&0.716&0.810&0.965 \tabularnewline
~~RMSE&0.663&0.661&0.596&0.625&0.658&0.719&0.813&0.967 \tabularnewline
\addlinespace[0.75ex]
\multicolumn{9}{l}{Estimand: ATE(RCT) = $-$0.001} \tabularnewline
\addlinespace[0.75ex]
~~Bias&0.663&0.558&0.564&0.616&0.653&0.716&0.811&0.965 \tabularnewline
~~RMSE&0.664&0.661&0.596&0.625&0.659&0.720&0.813&0.967 \tabularnewline
\addlinespace[0.75ex]
\multicolumn{9}{l}{Estimand: LATE = 0.564} \tabularnewline
\addlinespace[0.75ex]
~~Bias&0.098&$-$0.007&$-$0.001&0.051&0.088&0.152&0.246&0.400 \tabularnewline
~~RMSE&0.101&0.354&0.194&0.122&0.126&0.167&0.254&0.405 \tabularnewline
\addlinespace[0.75ex]
\multicolumn{9}{l}{Estimand: LATE(RCT) = 0.566} \tabularnewline
\addlinespace[0.75ex]
~~Bias&0.096&$-$0.009&$-$0.003&0.048&0.086&0.149&0.244&0.398 \tabularnewline
~~RMSE&0.099&0.354&0.194&0.121&0.124&0.165&0.252&0.403 \tabularnewline
\addlinespace[0.75ex]
SD&0.021&0.354&0.194&0.111&0.090&0.070&0.062&0.060 \tabularnewline
\addlinespace[0.75ex]
Coverage&0.4\%&95.2\%&94.4\%&92.7\%&84.0\%&46.0\%&3.1\%&0.0\% \tabularnewline
\addlinespace[0.75ex]
Avg N&10000&100&397&1175&1722&2613&3349&3994 \tabularnewline
\addlinespace[1.5ex]
\multicolumn{9}{c}{Panel B: Heterogeneous Conditional Effects (Model B)} \tabularnewline
\addlinespace[1.5ex]
\multicolumn{9}{l}{Estimand: ATE = 0} \tabularnewline
\addlinespace[0.75ex]
~~Bias&1.010&0.541&0.470&0.491&0.521&0.589&0.696&0.883 \tabularnewline
~~RMSE&1.010&0.667&0.519&0.507&0.532&0.594&0.700&0.885 \tabularnewline
\addlinespace[0.75ex]
\multicolumn{9}{l}{Estimand: ATE(RCT) = $-$0.004} \tabularnewline
\addlinespace[0.75ex]
~~Bias&1.014&0.546&0.474&0.496&0.526&0.593&0.701&0.887 \tabularnewline
~~RMSE&1.014&0.670&0.523&0.512&0.536&0.599&0.704&0.890 \tabularnewline
\addlinespace[0.75ex]
\multicolumn{9}{l}{Estimand: LATE = 0.564} \tabularnewline
\addlinespace[0.75ex]
~~Bias&0.446&$-$0.023&$-$0.094&$-$0.073&$-$0.042&0.025&0.132&0.319 \tabularnewline
~~RMSE&0.446&0.390&0.240&0.146&0.112&0.084&0.150&0.325 \tabularnewline
\addlinespace[0.75ex]
\multicolumn{9}{l}{Estimand: LATE(RCT) = 0.559} \tabularnewline
\addlinespace[0.75ex]
~~Bias&0.450&$-$0.018&$-$0.090&$-$0.068&$-$0.038&0.029&0.137&0.323 \tabularnewline
~~RMSE&0.451&0.390&0.238&0.144&0.110&0.085&0.154&0.330 \tabularnewline
\addlinespace[0.75ex]
SD&0.018&0.389&0.221&0.127&0.104&0.080&0.071&0.065 \tabularnewline
\addlinespace[0.75ex]
Coverage&0.0\%&94.6\%&92.4\%&91.7\%&94.1\%&93.5\%&51.8\%&0.3\% \tabularnewline
\addlinespace[0.75ex]
Avg N&10000&100&397&1175&1722&2613&3349&3994 \tabularnewline
\bottomrule %\addlinespace[1.5ex]

\end{tabularx}
\caption*{
\scriptsize {\it Note}: This table shows the bias, root mean squared error (RMSE), and standard deviation (SD) of OLS with no controls, 2SLS with $A(X_i)$ controls, and 2SLS with Approximate Propensity Score controls. These statistics are computed with the estimand set to ATE, ATE(RCT), LATE, or LATE(RCT). The ``Coverage'' row  in each panel shows the probabilities that the 95\% confidence intervals of the form $[\hat\beta_1^{s}-1.96\hat\sigma_n^{s},\hat\beta_1^{s}+1.96\hat\sigma_n^{s}]$ contains LATE(RCT), where $\hat\beta_1^{s}$ is the estimate and $\hat\sigma_n^{s}$ is its heteroskedasticity-robust standard error. We use 1,000 replications of a size 10,000 simulated sample to compute these statistics. We use several possible values of $\delta$ to compute the Approximate Propensity Score. All Approximate Propensity Scores are computed by averaging 400 simulation draws of $A(X_i)$. Panel A reports the results under the model in which the treatment effect does not depend on $X_i$ (Model A). Panel B reports the results under the model in which the treatment effect depends on $X_i$ (Model B). The bottom row  in each panel shows the average number of observations used for estimation (i.e., the average number of observations for which the Approximate Propensity Score or $A(X_i)$ is strictly between 0 and 1).
}
}
\label{table:simulation_rf_old}
\end{table}
%\restoregeometry


==> tables/simulation_10k.tex <==
\newgeometry{margin=0.95in}

\begin{table}[bp] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Comparison of Estimators and Coverage of Confidence Intervals}
{\scriptsize
\begin{tabularx}{\textwidth}{lCCCCCCCC}

\toprule
{}&{}&{}&\multicolumn{6}{c}{Our Method: 2SLS with Approximate Propensity Score Controls} \tabularnewline {}&{OLS}&{2SLS}&\tabularnewline[-2.5ex] \cline{4-9} \tabularnewline
{}&{with No Controls}&{with $A(X_i)$ Controls}&{$\delta = 0.01$}&{$\delta = 0.05$}&{$\delta = 0.1$}&{$\delta = 0.25$}&{$\delta = 0.5$}&{$\delta = 1$} \tabularnewline
\midrule\addlinespace[1.5ex]
\multicolumn{9}{c}{Panel A: Homogeneous Conditional Effects (Model A)} \tabularnewline
\addlinespace[1.5ex]
\multicolumn{9}{l}{Estimand: ATE = 0} \tabularnewline
\addlinespace[0.75ex]
~~Median Bias&0.663&0.566&0.569&0.616&0.651&0.715&0.808&0.963 \tabularnewline
~~Median Absolute Error&0.663&0.568&0.569&0.616&0.651&0.715&0.808&0.963 \tabularnewline
\addlinespace[0.75ex]
\multicolumn{9}{l}{Estimand: ATE(RCT) = $-$0.001} \tabularnewline
\addlinespace[0.75ex]
~~Median Bias&0.664&0.567&0.570&0.617&0.651&0.716&0.808&0.964 \tabularnewline
~~Median Absolute Error&0.664&0.569&0.570&0.617&0.651&0.716&0.808&0.964 \tabularnewline
\addlinespace[0.75ex]
\multicolumn{9}{l}{Estimand: LATE = 0.564} \tabularnewline
\addlinespace[0.75ex]
~~Median Bias&0.099&0.002&0.005&0.052&0.086&0.151&0.244&0.399 \tabularnewline
~~Median Absolute Error&0.099&0.238&0.131&0.084&0.092&0.151&0.244&0.399 \tabularnewline
\addlinespace[0.75ex]
\multicolumn{9}{l}{Estimand: LATE(RCT) = 0.566} \tabularnewline
\addlinespace[0.75ex]
~~Median Bias&0.097&0.000&0.003&0.050&0.084&0.149&0.241&0.396 \tabularnewline
~~Median Absolute Error&0.097&0.239&0.131&0.083&0.090&0.149&0.241&0.396 \tabularnewline
\addlinespace[0.75ex]
Med. Abs. Deviation from Median&0.014&0.239&0.131&0.076&0.062&0.048&0.043&0.041 \tabularnewline
\addlinespace[0.75ex]
Avg N&10000&100&397&1175&1723&2612&3348&3995 \tabularnewline
\addlinespace[1.5ex]
\multicolumn{9}{c}{Panel B: Heterogeneous Conditional Effects (Model B)} \tabularnewline
\addlinespace[1.5ex]
\multicolumn{9}{l}{Estimand: ATE = 0} \tabularnewline
\addlinespace[0.75ex]
~~Median Bias&1.010&0.557&0.478&0.497&0.523&0.589&0.695&0.883 \tabularnewline
~~Median Absolute Error&1.010&0.560&0.478&0.497&0.523&0.589&0.695&0.883 \tabularnewline
\addlinespace[0.75ex]
\multicolumn{9}{l}{Estimand: ATE(RCT) = $-$0.004} \tabularnewline
\addlinespace[0.75ex]
~~Median Bias&1.015&0.561&0.483&0.501&0.527&0.593&0.699&0.887 \tabularnewline
~~Median Absolute Error&1.015&0.564&0.483&0.501&0.527&0.593&0.699&0.887 \tabularnewline
\addlinespace[0.75ex]
\multicolumn{9}{l}{Estimand: LATE = 0.564} \tabularnewline
\addlinespace[0.75ex]
~~Median Bias&0.446&$-$0.007&$-$0.086&$-$0.067&$-$0.041&0.025&0.131&0.319 \tabularnewline
~~Median Absolute Error&0.446&0.256&0.156&0.098&0.075&0.057&0.131&0.319 \tabularnewline
\addlinespace[0.75ex]
\multicolumn{9}{l}{Estimand: LATE(RCT) = 0.559} \tabularnewline
\addlinespace[0.75ex]
~~Median Bias&0.451&$-$0.002&$-$0.081&$-$0.062&$-$0.037&0.029&0.136&0.324 \tabularnewline
~~Median Absolute Error&0.451&0.257&0.155&0.096&0.074&0.058&0.136&0.324 \tabularnewline
\addlinespace[0.75ex]
Med. Abs. Deviation from Median&0.013&0.257&0.145&0.085&0.070&0.054&0.049&0.045 \tabularnewline
\addlinespace[0.75ex]
Avg N&10000&100&397&1175&1723&2612&3348&3995 \tabularnewline
\bottomrule 

\end{tabularx}
\caption*{
\scriptsize {\it Note}: This table shows the median bias, median of absolute errors, and median of absolute deviations from the median estimate of OLS with no controls, 2SLS with $A(X_i)$ controls, and 2SLS with Approximate Propensity Score controls. These statistics are computed with the estimand set to ATE, ATE(RCT), LATE, or LATE(RCT). We use 10,000 replications of a size 10,000 simulated sample to compute these statistics. We use several possible values of $\delta$ to compute the Approximate Propensity Score. All Approximate Propensity Scores are computed by averaging 400 simulation draws of $A(X_i)$. Panel A reports the results under the model in which the treatment effect does not depend on $X_i$ (Model A). Panel B reports the results under the model in which the treatment effect depends on $X_i$ (Model B). The bottom row  in each panel shows the average number of observations used for estimation (i.e., the average number of observations for which the Approximate Propensity Score or $A(X_i)$ is strictly between 0 and 1).}
}
% \label{table:simulation_rf}
\end{table}

\restoregeometry


==> tables/simulation_het.tex <==
\newgeometry{margin=0.95in}

\begin{table}[bp] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Median Bias and Quantiles of Deviation for Estimators: Heterogeneous Conditional Effects (Model B)}
{\scriptsize
\begin{tabularx}{\textwidth}{lCCCCCCCC}

\toprule
{}&{}&{}&\multicolumn{6}{c}{Our Method: 2SLS with Approximate Propensity Score Controls} \tabularnewline {}&{OLS}&{2SLS}&\tabularnewline[-2.5ex] \cline{4-9} \tabularnewline
{}&{with No Controls}&{with $A(X_i)$ Controls}&{$\delta = 0.01$}&{$\delta = 0.05$}&{$\delta = 0.1$}&{$\delta = 0.25$}&{$\delta = 0.5$}&{$\delta = 1$} \tabularnewline
\midrule\addlinespace[1.5ex]
\multicolumn{9}{l}{Estimand: ATE = 0} \tabularnewline
\addlinespace[0.75ex]
~~Median Bias&1.010&0.561&0.471&0.496&0.525&0.590&0.698&0.882 \tabularnewline
~~Deviation Quantile $0.10$&0.986&0.146&0.184&0.325&0.393&0.487&0.605&0.804 \tabularnewline
~~Deviation Quantile $0.25$&0.997&0.295&0.311&0.407&0.451&0.537&0.650&0.839 \tabularnewline
~~Deviation Quantile $0.50$&1.010&0.566&0.471&0.496&0.525&0.590&0.698&0.882 \tabularnewline
~~Deviation Quantile $0.75$&1.022&0.803&0.621&0.576&0.591&0.642&0.741&0.927 \tabularnewline
~~Deviation Quantile $0.90$&1.032&1.003&0.748&0.651&0.649&0.690&0.786&0.967 \tabularnewline
\addlinespace[0.75ex]
\multicolumn{9}{l}{Estimand: ATE(RCT) = $-$0.004} \tabularnewline
\addlinespace[0.75ex]
~~Median Bias&1.015&0.566&0.475&0.500&0.529&0.595&0.702&0.887 \tabularnewline
~~Deviation Quantile $0.10$&0.990&0.148&0.188&0.329&0.397&0.491&0.610&0.809 \tabularnewline
~~Deviation Quantile $0.25$&1.001&0.299&0.316&0.412&0.455&0.542&0.655&0.843 \tabularnewline
~~Deviation Quantile $0.50$&1.015&0.571&0.475&0.500&0.529&0.595&0.702&0.887 \tabularnewline
~~Deviation Quantile $0.75$&1.026&0.808&0.625&0.581&0.596&0.646&0.746&0.931 \tabularnewline
~~Deviation Quantile $0.90$&1.037&1.007&0.752&0.655&0.653&0.695&0.790&0.972 \tabularnewline
\addlinespace[0.75ex]
\multicolumn{9}{l}{Estimand: LATE = 0.564} \tabularnewline
\addlinespace[0.75ex]
~~Median Bias&0.446&$-$0.002&$-$0.093&$-$0.068&$-$0.039&0.026&0.134&0.318 \tabularnewline
~~Deviation Quantile $0.10$&0.422&0.046&0.031&0.019&0.013&0.009&0.043&0.240 \tabularnewline
~~Deviation Quantile $0.25$&0.433&0.128&0.077&0.048&0.034&0.027&0.086&0.275 \tabularnewline
~~Deviation Quantile $0.50$&0.446&0.262&0.163&0.099&0.073&0.057&0.134&0.318 \tabularnewline
~~Deviation Quantile $0.75$&0.458&0.421&0.285&0.166&0.132&0.092&0.177&0.363 \tabularnewline
~~Deviation Quantile $0.90$&0.468&0.649&0.396&0.241&0.184&0.139&0.222&0.403 \tabularnewline
\addlinespace[0.75ex]
\multicolumn{9}{l}{Estimand: LATE(RCT) = 0.559} \tabularnewline
\addlinespace[0.75ex]
~~Median Bias&0.451&0.002&$-$0.089&$-$0.063&$-$0.035&0.031&0.138&0.323 \tabularnewline
~~Deviation Quantile $0.10$&0.427&0.048&0.033&0.017&0.014&0.010&0.047&0.245 \tabularnewline
~~Deviation Quantile $0.25$&0.437&0.124&0.076&0.047&0.034&0.026&0.091&0.279 \tabularnewline
~~Deviation Quantile $0.50$&0.451&0.265&0.162&0.097&0.074&0.057&0.138&0.323 \tabularnewline
~~Deviation Quantile $0.75$&0.462&0.420&0.286&0.166&0.128&0.095&0.182&0.367 \tabularnewline
~~Deviation Quantile $0.90$&0.473&0.645&0.393&0.237&0.182&0.143&0.226&0.408 \tabularnewline
\addlinespace[0.75ex]
Deviation from Median Quantile $0.10$&0.002&0.047&0.029&0.016&0.012&0.010&0.010&0.009 \tabularnewline
Deviation from Median Quantile $0.25$&0.006&0.126&0.071&0.043&0.032&0.025&0.023&0.022 \tabularnewline
Deviation from Median Quantile $0.50$&0.012&0.264&0.153&0.084&0.071&0.052&0.045&0.044 \tabularnewline
Deviation from Median Quantile $0.75$&0.021&0.421&0.254&0.148&0.116&0.089&0.080&0.075 \tabularnewline
Deviation from Median Quantile $0.90$&0.030&0.647&0.371&0.209&0.171&0.132&0.118&0.108 \tabularnewline
\addlinespace[0.75ex]
Avg N&10000&100&397&1175&1722&2613&3349&3994 \tabularnewline
\bottomrule 

\end{tabularx}
\caption*{
\scriptsize {\it Note}: This table shows the median bias, quantiles for absolute deviation, and quantiles for absolute deviation from the median estimate of OLS with no controls, 2SLS with $A(X_i)$ controls, and 2SLS with Approximate Propensity Score controls. These statistics are computed with the estimand set to ATE, ATE(RCT), LATE, or LATE(RCT). We use 1,000 replications of a size 10,000 simulated sample to compute these statistics. We use several possible values of $\delta$ to compute the Approximate Propensity Score. All Approximate Propensity Scores are computed by averaging 400 simulation draws of $A(X_i)$. Panel A reports the results under the model in which the treatment effect does not depend on $X_i$ (Model A). Panel B reports the results under the model in which the treatment effect depends on $X_i$ (Model B). The bottom row  in each panel shows the average number of observations used for estimation (i.e., the average number of observations for which the Approximate Propensity Score or $A(X_i)$ is strictly between 0 and 1).}
}
%\label{table:simulation_rf}
\end{table}

\restoregeometry


==> tables/simulation_hom.tex <==
\newgeometry{margin=0.95in}

\begin{table}[bp] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\caption{Median Bias and Quantiles of Deviation for Estimators: Homogeneous Conditional Effects (Model A)}
{\scriptsize
\begin{tabularx}{\textwidth}{lCCCCCCCC}

\toprule
{}&{}&{}&\multicolumn{6}{c}{Our Method: 2SLS with Approximate Propensity Score Controls} \tabularnewline {}&{OLS}&{2SLS}&\tabularnewline[-2.5ex] \cline{4-9} \tabularnewline
{}&{with No Controls}&{with $A(X_i)$ Controls}&{$\delta = 0.01$}&{$\delta = 0.05$}&{$\delta = 0.1$}&{$\delta = 0.25$}&{$\delta = 0.5$}&{$\delta = 1$} \tabularnewline
\midrule\addlinespace[1.5ex]
\multicolumn{9}{l}{Estimand: ATE = 0} \tabularnewline
\addlinespace[0.75ex]
~~Median Bias&0.663&0.562&0.558&0.618&0.652&0.716&0.811&0.965 \tabularnewline
~~Deviation Quantile $0.10$&0.636&0.140&0.321&0.472&0.543&0.628&0.733&0.889 \tabularnewline
~~Deviation Quantile $0.25$&0.649&0.342&0.431&0.540&0.590&0.669&0.770&0.924 \tabularnewline
~~Deviation Quantile $0.50$&0.663&0.562&0.558&0.618&0.652&0.716&0.811&0.965 \tabularnewline
~~Deviation Quantile $0.75$&0.677&0.776&0.687&0.690&0.713&0.760&0.851&1.007 \tabularnewline
~~Deviation Quantile $0.90$&0.691&0.995&0.814&0.756&0.770&0.805&0.891&1.040 \tabularnewline
\addlinespace[0.75ex]
\multicolumn{9}{l}{Estimand: ATE(RCT) = $-$0.001} \tabularnewline
\addlinespace[0.75ex]
~~Median Bias&0.663&0.562&0.559&0.618&0.653&0.717&0.811&0.966 \tabularnewline
~~Deviation Quantile $0.10$&0.636&0.141&0.322&0.472&0.543&0.628&0.734&0.890 \tabularnewline
~~Deviation Quantile $0.25$&0.650&0.342&0.431&0.541&0.590&0.670&0.770&0.925 \tabularnewline
~~Deviation Quantile $0.50$&0.663&0.563&0.559&0.618&0.653&0.717&0.811&0.966 \tabularnewline
~~Deviation Quantile $0.75$&0.678&0.777&0.688&0.691&0.714&0.761&0.852&1.007 \tabularnewline
~~Deviation Quantile $0.90$&0.691&0.996&0.814&0.757&0.771&0.805&0.892&1.040 \tabularnewline
\addlinespace[0.75ex]
\multicolumn{9}{l}{Estimand: LATE = 0.564} \tabularnewline
\addlinespace[0.75ex]
~~Median Bias&0.098&$-$0.002&$-$0.006&0.053&0.088&0.152&0.246&0.401 \tabularnewline
~~Deviation Quantile $0.10$&0.071&0.036&0.025&0.016&0.017&0.064&0.169&0.325 \tabularnewline
~~Deviation Quantile $0.25$&0.085&0.097&0.061&0.039&0.044&0.105&0.206&0.360 \tabularnewline
~~Deviation Quantile $0.50$&0.098&0.222&0.129&0.084&0.091&0.152&0.246&0.401 \tabularnewline
~~Deviation Quantile $0.75$&0.113&0.402&0.220&0.142&0.150&0.196&0.287&0.442 \tabularnewline
~~Deviation Quantile $0.90$&0.126&0.568&0.321&0.202&0.206&0.240&0.327&0.475 \tabularnewline
\addlinespace[0.75ex]
\multicolumn{9}{l}{Estimand: LATE(RCT) = 0.566} \tabularnewline
\addlinespace[0.75ex]
~~Median Bias&0.096&$-$0.005&$-$0.008&0.051&0.086&0.150&0.244&0.399 \tabularnewline
~~Deviation Quantile $0.10$&0.069&0.038&0.024&0.016&0.016&0.062&0.167&0.323 \tabularnewline
~~Deviation Quantile $0.25$&0.083&0.098&0.062&0.039&0.043&0.103&0.203&0.358 \tabularnewline
~~Deviation Quantile $0.50$&0.096&0.223&0.129&0.083&0.089&0.150&0.244&0.399 \tabularnewline
~~Deviation Quantile $0.75$&0.111&0.402&0.220&0.142&0.148&0.194&0.285&0.440 \tabularnewline
~~Deviation Quantile $0.90$&0.124&0.568&0.319&0.202&0.204&0.238&0.325&0.473 \tabularnewline
\addlinespace[0.75ex]
Deviation from Median Quantile $0.10$&0.003&0.037&0.022&0.017&0.011&0.008&0.008&0.007 \tabularnewline
Deviation from Median Quantile $0.25$&0.006&0.098&0.060&0.035&0.029&0.020&0.021&0.019 \tabularnewline
Deviation from Median Quantile $0.50$&0.014&0.224&0.128&0.075&0.062&0.045&0.041&0.041 \tabularnewline
Deviation from Median Quantile $0.75$&0.024&0.403&0.219&0.126&0.103&0.079&0.070&0.070 \tabularnewline
Deviation from Median Quantile $0.90$&0.036&0.566&0.319&0.187&0.148&0.116&0.105&0.096 \tabularnewline
\addlinespace[0.75ex]
Avg N&10000&100&397&1175&1722&2613&3349&3994 \tabularnewline
\bottomrule 

\end{tabularx}
\caption*{
\scriptsize {\it Note}: This table shows the median bias, quantiles for absolute deviation, and quantiles for absolute deviation from the median estimate of OLS with no controls, 2SLS with $A(X_i)$ controls, and 2SLS with Approximate Propensity Score controls. These statistics are computed with the estimand set to ATE, ATE(RCT), LATE, or LATE(RCT). We use 1,000 replications of a size 10,000 simulated sample to compute these statistics. We use several possible values of $\delta$ to compute the Approximate Propensity Score. All Approximate Propensity Scores are computed by averaging 400 simulation draws of $A(X_i)$. Panel A reports the results under the model in which the treatment effect does not depend on $X_i$ (Model A). Panel B reports the results under the model in which the treatment effect depends on $X_i$ (Model B). The bottom row  in each panel shows the average number of observations used for estimation (i.e., the average number of observations for which the Approximate Propensity Score or $A(X_i)$ is strictly between 0 and 1).}
}
%\label{table:simulation_rf}
\end{table}

\restoregeometry

